Mobile Traffic Classification through Physical Channel Fingerprinting: a Deep Learning Approach

The automatic classification of applications and services is an invaluable feature for new generation mobile networks. Here, we propose and validate algorithms to perform this task, at runtime, from the raw physical channel of an operative mobile network, without having to decode and/or decrypt the transmitted flows. Towards this, we decode Downlink Control Information (DCI) messages carried within the LTE Physical Downlink Control CHannel (PDCCH). DCI messages are sent by the radio cell in clear text and, in this paper, are utilized to classify the applications and services executed at the connected mobile terminals. Two datasets are collected through a large measurement campaign: one labeled, used to train the classification algorithms, and one unlabeled, collected from four radio cells in the metropolitan area of Barcelona, in Spain. Among other approaches, our Convolutional Neural Network (CNN) classifier provides the highest classification accuracy of 99%. The CNN classifier is then augmented with the capability of rejecting sessions whose patterns do not conform to those learned during the training phase, and is subsequently utilized to attain a fine grained decomposition of the traffic for the four monitored radio cells, in an online and unsupervised fashion.

==> Mobile Data Analysis - Journal/Abstract.tex <==
%\IEEEtitleabstractindextext{
\begin{abstract} 
The automatic classification of applications and services is an invaluable feature for new generation mobile networks. Here, we propose and validate algorithms to perform this task, at {\it runtime}, from the {\it raw physical channel} of an {\it operative mobile network}, without having to decode and/or decrypt the transmitted flows. Towards this, we decode Downlink Control Information (DCI) messages carried within the LTE Physical Downlink Control CHannel (PDCCH). DCI messages are sent by the radio cell in clear text and, in this paper, are utilized to classify the applications and services executed at the connected mobile terminals. Two datasets are collected through a large measurement campaign: one labeled, used to train the classification algorithms, and one unlabeled, collected from four radio cells in the metropolitan area of Barcelona, in Spain. Among other approaches, our Convolutional Neural Network (CNN) classifier provides the highest classification accuracy of $99\%$. The CNN classifier is then augmented with the capability of rejecting sessions whose patterns do not conform to those learned during the training phase, and is subsequently utilized to attain a fine grained decomposition of the traffic for the four monitored radio cells, in an {\it online} and {\it unsupervised} fashion. 
\end{abstract}
 
%old abstract
%The automatic classification of applications and services is an invaluable feature for new generation mobile networks. Here, we are concerned with effectively performing this classification task, at {\it runtime}, from the {\it raw physical channel} of an {\it operative mobile network}. As a first step towards this, we have built a platform to monitor the LTE Physical Downlink Control CHannel (PDCCH). Downlink Control Information (DCI) messages are sent unencrypted within the PDCCH and, from them, temporal information about the allocated Resource Blocks (RBs), Modulation and Coding Scheme (MCS) and Transport Block Size (TBS) for the active users within the monitored radio cell is extracted. From DCI data two datasets are obtained: one is {\it labeled}, thanks to the injection of a watermark into mobile app flows, which can be easily identified and, in turn, utilized to identify the traffic produced by a device under our control. The second dataset is {\it unlabeled}, and contains DCI session data with Transmission Time Interval (TTI) granularity from four radio cell sites of a Spanish operative mobile network, where each site has been monitored for a full month. Traffic classifiers based on Multi-Layer Perceptrons (MLPs), Convolutional (CNN) and Recurrent (RNN) Neural Networks, as well as on Support Vector Machines (SVMs), Gaussian Processes (GP), and Random Forests (RF), are tailored to the considered problem, and trained in a supervised manner using the labeled dataset. CNNs provide the highest classification accuracy, ranging from $97.8$ to $99\%$, and reach an $F$-Score of $0.97$ and $0.98$ for application and service identification tasks, respectively. Most importantly, an original technique is presented to augment the CNN classifier with the capability of rejecting out of distribution (OOD) sessions, i.e., sessions whose patterns do not conform to those learned during the training phase. This augmented CNN is then utilized to attain a fine grained decomposition of the traffic for the four monitored radio cells, in an {\it online} and {\it unsupervised} fashion.   

%With the purpose to make next generation networks aware of the traffic they are serving and of the users' behaviors, in this paper, we target traffic classification and profiling based on real raw data extracted from an operative network. Without loss of generality with respect to the services, applications and network considered, we present a methodology that is able to classify with extremely high accuracy (up to 99 \%) the service and applications based on raw physical layer data, directly extracted from a Long Term Evolution (LTE) commercial network.
%	The methodology that we propose consists of five steps. First, we build a platform to directly monitor the unencrypted Physical Downlink Control CHannel (PDCCH), where Downlink Control Information (DCI) messages are exchanged. DCIs contain, among others, information about allocated Resource Blocks (RBs) and Modulation and Coding Scheme (MCS). Second, we monitor four cells in four demographically different areas in Barcelona, Spain, each for a periodo of one month. With this data, we are able to build an unlabeled database with Transmission Time Interval (TTI) granularity. Third, we perform multiple experiments, by injecting and then tracking data from known applications and build a labeled database, for training purposes. Fourth, we build multiple deep architectures to learn in supervised way the proper service and application classification.  We test the classifiers on the labeled database, obtaining high levels of accuracy. We study the performance of the deep neural network architectures against more traditional Machine Learning (ML) solutions, demonstrating the superiority of deep solutions. Finally, we perform service classification on the unlabeled database, resulting in a high granularity traffic profiling during the 24 hours of a day, capable of characterizing mobile usage patterns in the different studied regions. The results confirm the accuracy of the proposed approach, after \mbox{cross-validation} with other approaches using data of other nature and methodologies. 
	
%TBR - Providing mobile networks with the capability to predict user behaviors is key to accomplish with the demanding requirements raised from the next generation of mobile networks. In this paper we present a framework to classify mobile traffic, which processes raw data from the \ac{LTE} radio interface. Specifically, we first present a methodology to collect user data by directly monitoring the \ac{PDCCH}, exploiting \ac{DCI} messages from multiple operative cells in Spain, and characterized by a variety of traffic loads and conditions. \ac{DCI} messages contain the network scheduling information, and allow us to know the assignation of the resource elements for each \ac{LTE} subframe by the eNodeB, among the contending \ac{UE}s. 

%Next, we disclose a procedure to identify a certain user associated to a monitored terminal among all users within the monitored eNodeB and to extract the mobile user sessions. Finally, an exhaustive benchmark is given to compare the performance of two supervised classification problems: service, and \ac{app} classification. To this end, we start from \mbox{state-of-the-art} supervised learning algorithms, and then we propose customized solutions based on \acp{NN}. Numerical results show that the \acp{NN} architectures overcome the other approaches in terms of classification accuracy. Moreover, we discuss practical applications and benefits that can arise from the use of this framework.



% Note that keywords are not normally used for peerreview papers.
\begin{IEEEkeywords}
Traffic Classification, Traffic Modeling, Mobile Networks, LTE, 5G, Machine Learning, Neural Networks, Deep Learning, Data Analytics. 
\end{IEEEkeywords}

%}




==> Mobile Data Analysis - Journal/Classification_Problem.tex <==
\section{Classification Problem}
\label{sec:sl}

\subsection{Problem Definition}
\label{sec:problem}

%Classification is the process of predicting the class of a given set of data. It belongs to the category of supervised learning where we can assign a label to each class.

%Let $\bm{X}$ be the $M \times N$ matrix representing the labeled dataset. Its \mbox{$m$-th} row vector $\bm{x}_m$ contains the trace associated with the \mbox{$m$-th} \ac{RNTI}, $M$ is the number of monitored \acp{RNTI} (here referred to as sessions) and $N$ is the number of \ac{TBS} samples per session.\footnote{Here, a TBS sample for a given session is obtained averaging the corresponding TBS measurements within a time window of $1$~s.} 
Let $M$ be the number of windowed-sessions obtained through the data preparation procedure of Section~\ref{sec:labeled_dataset}, $W$ is the window size, and $D = 2$ is the number of communication directions (downlink and uplink). We define $\bm{X}$ the input dataset tensor with size $M \times W \times D$, where the \mbox{$m$-th} row vector $\bm{x}_m$ contains the trace associated with $W$ \ac{TBS} samples per session for both downlink and uplink directions ($D=2$).

A classifier estimates a function $c:\bm{X} \rightarrow \bm{Y}$, where the output matrix $\bm{Y}$ has size $M \times K$, with $K$ representing the number of classes. The row vector \mbox{$\bm{y_m}=c(\bm{x_m})=[y_{m1},\dots, y_{mK}]$} contains the probabilities that session $m$ belongs to each of the $K$ classes, with $\sum_{k} y_{mk} =1$. The final output of the classifier is class $k^\star$, where $k^\star = \arg\!\max_k (y_{mk})$. The following classification objectives are addressed:
\begin{enumerate}
	\item[O1)] \textbf{Service identification:} to classify the collected sessions into $K = 3$ classes, namely, {\it audio streaming}, {\it video streaming} and {\it video calls};
	\item[O2)] \textbf{App identification:} to identify which app is run at the \ac{UE}. In this case, the number of output classes is $K=6$, namely, \textit{Spotify}, \textit{Google Music}, \textit{YouTube}, \textit{Vimeo}, \textit{Skype} and \textit{WhatsApp Messenger}.
\end{enumerate}

%In our framework, the labeled dataset can be expressed as:
%\begin{equation}
%\bm{X} = \{\bm{x_m} \mid m = 1,\dots, M\}
%\end{equation}
%where $\bm{x_m}$ is the trace associated with the $m$-th RNTI and characterized by a fixed length of $N$ TBS samples, being a sample the average TBS observed in $1$ s. $M=10000$ is the total number of monitored RNTIs (hereinafter also referred to as sessions). Since all traces have equal duration, i.e., the same number of samples per session, the whole labeled dataset $\bm{X}$ is an $M \times N$ matrix and will be used as the input of the classification problem.
%Formally, a classifier estimates a function $c:\bm{X} \rightarrow \bm{Y}$, where $ \bm{Y} = \{y_m \mid m = 1,\dots, M\}$. The output is then a stochastic vector $\bm{y_m} = c(\bm{x_m})$, where the $k$-th entry $y_k$ of $\bm{y_m}$ is the probability that the trace corresponds to the $k$-th class. As for the input $\bm{X}$, we define $\bm{Y}$ as the output $M\times K$ matrix containing the probabilistic output $\bm{y_m}$ of the classifiers. The output class is the $k$-th class that has the highest probability, computed as $arg\,max_k (\bm{y_m})$.

Next, we present the considered classification algorithms, grouping them into two categories: those based on artificial neural networks and those based on standard machine learning techniques (referred to here as benchmark classifiers). 
%Formally, given a set of classifiers $\mathcal{C}=\{c_i \mid i=1\dots C\}$, each classifier is a function $c:\bm{X} \rightarrow \bm{K}$, which outputs for each session the probability that this session belongs to a class for that problem and where $ \bm{K} = \{y_m \mid m = 1,\dots, M\}$. The output is then a stochastic vector $\bm{y_m} = c(\bm{x_m})$, where the $k$-th entry $y_k$ of $\bm{y_m}$ is the probability that the trace corresponds to the $k$-th class ($K=\{3,6\}$). As for the input $\bm{X}$, we define $\bm{Y}$ as the output $M\times K$ matrix containing the probabilistic output $\bm{y_m}$ of the classifiers. The output class is the $k$-th class that has the highest probability, computed as $arg\,max_k (\bm{y_m})$.
%More details about the classifiers used in solving the two problems are given in Sections~\ref{sec:sl} and \ref{sec:nn}.


\subsection{Deep Neural Networks}
\label{sec:nn}

Next, we describe how we tailored three neural network architectures to solve the above traffic classification problem, namely,  \ac{MLP}, Recurrent Neural Networks (RNNs) and Convolutional Neural Networks (CNNs). 

%Details about the customized architectures are provided in the next subsections. It should be noted that the layer settings provided for each \ac{NN} are specific for the obtained dataset explained in Section~\ref{sec:dataset}, with the goal of obtaining the highest performance in terms of accuracy, with the lowest complexity. In contrast to methods presented in Section~\ref{sec:benchmark}, these tools enable automatic feature detection within the raw dataset traces, which provides an improvement in the classification performance as we will show in Section~\ref{sec:results}.

\subsubsection{Multilayer Perceptron}
\label{sec:nn_mlp}

A multilayer perceptron is a feedforward and \mbox{fully-connected} neural network architecture. The term \mbox{``feed-forward''} refers to the fact that the information flows in one direction, from the input to the output layer. An MLP is composed of, at least, three layers of nodes: an input, a hidden and an output layer. A directed graph connects the input with the output layer and each neuron in the graph uses a \mbox{non-linear} activation function to produce its output. Links are weighted and the backpropagation algorithm is utilized to train the network in a supervised fashion, i.e., to find the set of network weights that minimize a certain error function, given an input set of examples and the corresponding labels. For further details, see~\cite{bishop2006}.

The \ac{MLP} that we use for mobile traffic classification has \emph{three} fully connected layers. The first layer ${MLP}_1$ contains $N_{{MLP}_1}= 128$ neurons, the second layer ${MLP}_2$ has $N_{{MLP}_2}= 64$ neurons and the third layer $MLP_3$ is fully connected, with $K$ neurons and a softmax activation function to produce the final output. The output of ${MLP}_3$ is the class probability vector $\bm{y_m}$.%: its \mbox{$k$-th} element can be interpreted as the probability that the input data belongs to class $k$, with $k = 1,2,\dots,K$. 

%It is common to The ReLU activation function is often used in neural network architectures and allows the activation to be thresholded at zero. However, during the training, large gradient flows through a ReLU neuron can cause the weights to update in such a way that the neuron will never activate on any data point again. If this happens, then the gradient flowing through the unit will forever be zero from that point on, and the neuron will be useless. Leaky \acp{ReLU} attempt to solve this, by forcing the function to have a small negative slope rather than zero value. The leaky \ac{ReLU} activation function has been used due to the need of tackling \mbox{non-linearities} present in the dataset. 
%Given an input $x$, Leaky ReLU is defined as:
%
%\begin{equation}
%f(x) = \left\{ 	\begin{array}{lr} 	\alpha x & : x < 0\\ 	x & : x \ge 0 	\end{array} \right.
%\end{equation}

%\noindent where $\alpha$ controls the negative slope and usually takes values around $0.1$.
%Moreover, the use of only linear activation functions in every layer would imply that the final activation function of the last layer would be just a linear function of the first input layer. This means that several layers can be replaced by a single layer, losing the ability of stacking layers and its improvement in finding hidden features within the input dataset.
%Finally, each output neuron in the last layer ${MLP}_3$ corresponds to a specific class $k \in K$.%, where $K=6$ classes for app classification and $K=3$ for service classification.
All neurons in layers $MLP_1$ and $MLP_2$ use a leaky version of the \ac{ReLU} ({\it leaky \ac{ReLU}}) activation function. Leaky \acp{ReLU} help solve the vanishing gradient problem, i.e., the fact that the error gradients that are backpropagated during the training of the network weights may become very small (zero in the worst case), preventing the correct (gradient based) adaptation of the weights. To prevent this from happening, leaky \acp{ReLU} have a small negative slope for negative values of their argument~\cite{maas2013rectifier}.
%, i.e., $y_{mk} = y_{mk}(\bm{w}) = Prob(t_k = 1|\bm{w})$, where $\bm{w}$ is the vector containing the \ac{MLP} weights of every layer and $\bm{t}=[t_1,\dots, t_K]$ is a vector whose elements are defined as $t_k = 1$ if $\bm{x_m}$ belongs to class $k$ and $t_k = 0$ otherwise. 
To train the presented MLP architecture, we use the {\it RMSprop} gradient descent algorithm~\cite{tieleman2012lecture}, by minimizing the {\it categorical \mbox{cross-entropy} loss function} $L(\bm{w})$, defined as~\cite{bishop2006} %(Eq. (5.24) of Section 5.2): 
\begin{equation}
\label{eq:cross}
L(\bm{w}) = - \sum_{\bm{x}_m \in \bm{B}} \sum_{k=1}^{K} t_k(\bm{x}_m) \log(y_{mk}(\bm{w}, \bm{x}_m)).
\end{equation}
where $\bm{t(x)_m} = [t_1(\bm{x}_m), \dots, t_k(\bm{x}_m)]$ contains the class labels associated with the input trace $\bm{x}_m$, i.e., $t_k=1$ if $\bm{x}_m$ belongs to class $k$ and $t_k = 0$ otherwise (\mbox{$1$-of-$K$} coding scheme). Vector $\bm{w}$ contains the \ac{MLP} weights and $y_{mk}(\bm{w}, \bm{x}_m)$ is the MLP output obtained for input $\bm{x}_m$. Eq.~(\ref{eq:cross}) is iteratively minimized using the training examples in the batch set $\bm{B}\subset \bm{X}$, where $\bm{B}$ is changed at every iteration so as to span the entire input set $\bm{X}$.

%If $\bm{X}$ is the set of all training examples, we define the batch set as $\bm{B} \subset \bm{X}$. Let $\bm{x_m} \in \bm{B}$ and denote the corresponding output vector by $\bm{y_m}(\bm{w})$ and its $k$-th entry by $y_{mk}(\bm{w})$, where $\bm{w}$ is the vector containing the \ac{MLP} weights of every layer. The corresponding target vector is $\bm{t(x_m)} = [t_1(\bm{x_m}), \dots, t_k(\bm{x_m})]$ \cite{gadaleta2016idnet} whose elements are defined as $t_k = 1$ if $\bm{x_m}$ belongs to class $k$ and $t_k = 0$ otherwise. The network is trained solving a \mbox{multi-class} classification problem using the {\it RMSprop} algorithm~\cite{tieleman2012lecture}, a specific gradient descend algorithm which minimizes a categorical \mbox{cross-entropy} loss function $L(\bm{w})$, defined as \cite{bishop2006} (Eq. (5.24) of Section 5.2):

%The output vectors of all layers have binary entries and are \mbox{hot-encoded}, i.e., all values are zero except for the entry corresponding to the output chosen class. The output of layer ${MLP}_3$ is a stochastic vector $\bm{y_m}$ obtained by a softmax activation function, whose $k$-th entry $k = 1,2,\dots,K$ can be seen as the probability that the input pattern belongs to class $k$, i.e., $y_k = y_k(\bm{w},\bm{x_m}) = Prob(t_k = 1|\bm{w},\bm{x_m})$, where $\bm{w}$ is the vector containing all the \ac{MLP} weights, $\bm{x_m}$ is the current input and $t_k = 1$ if $\bm{x_m}$ belongs to class $k$ and $t_k = 0$ otherwise. If $\bm{X}$ is the set of all training examples, we define the batch set as $\bm{B} \subset \bm{X}$. Let $\bm{x_m} \in \bm{B}$ and denote the corresponding output vector by $\bm{y_m}(\bm{w},\bm{x_m})$ and its $k$-th entry by $y_k(\bm{w},\bm{x_m})$. The corresponding target vector is $\bm{t(x_m)} = (t_1(\bm{x_m}), \dots, t_k(\bm{x_m}))^T$ \cite{gadaleta2016idnet}. The network is trained in a supervised manner solving a \mbox{multi-class} classification problem using the {\it RMSprop} algorithm~\cite{tieleman2012lecture}, a specific gradient descend algorithm which minimizes a categorical \mbox{cross-entropy} loss function $L(\bm{w})$, defined as \cite{bishop2006} (Eq. (5.24) of Section 5.2):

%\begin{equation}
%\label{eq:cross}
%L(\bm{w}) = - \sum_{\bm{x_m} \in \bm{B}} \sum_{k=1}^{K} t_k(\bm{x_m}) log(y_{mk}(\bm{w})).
%\end{equation}

\subsubsection{Recurrent Neural Networks}
\label{sec:nn_rnn}

Recurrent Neural Networks (RNNs) have been conceived to extract features from temporal (and correlated) data sequences. \ac{LSTM} networks are a particular type of \ac{RNN}, introduced in \cite{Hochreiter1997}. They are capable of tracking \mbox{long-term} dependencies into the input time series, while solving the \mbox{vanishing-gradient} problem that affects standard \acp{RNN}~\cite{gers1999learning}.

The capability of learning \mbox{long-term} dependencies is due to the structure of the \ac{LSTM} cells, which incorporates gates that regulate the learning process. The neurons in the hidden layers of an \ac{LSTM} are \acp{MC}. A \ac{MC} has the ability to retain or forget information about past input values (whose effect is stored into the cell states) by using structures called {\it gates}, which consist of a cascade of a neuron with sigmoidal activation function and a pointwise multiplication block. Thanks to this architecture, the output of each memory cell possibly depends on the entire sequence of past states, making \acp{LSTM} suitable for processing time series with long time dependencies~\cite{Hochreiter1997}. The input gate of a memory cell is a neuron with sigmoidal activation function ($\sigma$). Its output determines the fraction of the MC input that is fed to the cell state block. Similarly, the forget gate processes the information that is recurrently fed back into the cell state block. The output gate, instead, determines the fraction of the cell state output that is to be used as the output of the \ac{MC}, at each time step. Gate neurons usually have sigmoidal activation functions ($\sigma$), while the hyperbolic tangent ($\tanh$) activation function is usually adopted to process the input and for the cell state. All the internal connections of the \ac{MC} have unitary weight~\cite{Hochreiter1997}.


\begin{figure}[t]	
	\centering
	\includegraphics[width=.8\columnwidth]{figures/lstm-eps-converted-to}
	\caption{\ac{RNN} architecture.}
	\label{fig:lstm_nn}	
\end{figure}

The proposed RNN based traffic classification architecture is shown in Fig.~\ref{fig:lstm_nn}. In our design, we consider three stacked layers combining two LSTM layers and a final fully connected output layer. The first and the second layer (respectively ${RNN}_1$ and ${RNN}_2$) have \mbox{$N_{{RNN}_1}=N_{{RNN}_2}= 180$} memory cells. The fully connected layer ${RNN}_3$ uses the softmax activation function and its output consists of the class probability estimates, as described in Section~\ref{sec:nn_mlp}.
%performs the actual \mbox{multi-class} classification as the final layer in the \ac{MLP} network. Hence, the explanation given in \ref{sec:nn_mlp} about it also applies here. Moroever, the same optimizer to minimize Eq.~\ref{eq:cross} has been used in this case.

%\begin{figure}[t]	
%	\centering
%	\includegraphics[width=\columnwidth]{figures/cnn.eps}
%	\caption{\angel{\ac{CNN} architecture.}}
%	\label{fig:cnn}	
%\end{figure}

\subsubsection{Convolutional Neural Networks}
\label{sec:nn_cnn}

\begin{figure}[t]	
	\centering
	\includegraphics[width=.8\columnwidth]{figures/cnn_2-eps-converted-to}
	\caption{\ac{CNN} architecture.}
	\label{fig:cnn}	
\end{figure}

Convolutional Neural Networks (CNNs) are \mbox{feed-forward} deep neural networks differing from fully connected MLP for the presence of one or more convolutional layers. At each convolutional layer, a number of kernels is used. Each kernel is composed of a number of weights and is convolved across the entire input signal. Note that the kernel acts as a filter whose weights are \mbox{re-used} ({\it shared weights}) across the entire input and this makes the network connectivity structure sparse, i.e., a small set of parameters (the kernel weights) suffices to map the input into the output. This leads to a considerably reduced computational complexity with respect to fully connected feed forward neural
networks, and to a smaller memory footprint. For more details the reader is referred to~\cite{goodfellow2016deep}. 

\acp{CNN} have been proven to be excellent feature extractors for images and inertial signals~\cite{gadaleta2016idnet} and here we show their effectiveness for the classification of mobile traffic data. The \ac{CNN} architecture that we designed to this purpose is shown in Fig.~\ref{fig:cnn}. It has two main parts: the first four layers perform convolutions and max pooling in cascade, the last two are fully connected layers. 
%It is composed of a cascade of two convolutional layers, followed by a pooling layer respectively, and finally a  \mbox{two-layer} fully connected network. The convolutional layers, in combination with the first fully connected layer, perform a dimensionality reduction (or automatic feature extraction) task, whereas the last fully connected one performs the \mbox{multi-class} classification. 
The first convolutional layer $CNN_1$ uses one dimensional kernels ($ 1\times 5$ samples) performing a first filtering of the input and processing each input vector (rows of $\bm{X}$) separately. The activation functions are linear and the number of convolutional kernels is $N_{{CNN}_1}=32$. The second convolutional layer, $CNN_2$, uses one dimensional kernels ($1 \times 5$ samples) with \mbox{non-linear} hyperbolic tangents as activation functions, and the number of convolutional kernels is $N_{{CNN}_2}=64$.
Max pooling is separately applied to the outputs of $CNN_1$ and $CNN_2$ to reduce their dimensionality and increase the spatial invariance of features~\cite{gadaleta2016idnet}. In both cases, a \mbox{one-dimensional} pooling with a kernel of size $1 \times 3$ is performed. A third fully connected layer, $CNN_3$, performs dimensionality reduction and has $N_{{CNN}_3}=32$ neurons with Leaky \ac{ReLU} activation functions. This layer is used in place of a further convolutional layer to reduce the computation time, with a negligible loss in accuracy. The last (output) layer $CNN_4$ is fully connected with softmax activation functions, and returns the class probability estimates, see Sections~\ref{sec:nn_mlp}.

\subsection{Benchmark classifiers}
\label{sec:benchmark}

Other standard classification schemes have been tailored to the considered tasks O1 and O2. The selected algorithms are: \textit{Linear Logistic Regression}, \textit{$K$-Nearest Neighbours} and \textit{Linear SVM}, as examples of linear classifiers; \textit{Random Forest}, as an ensemble learning method, and \textit{Gaussian Processes} as an instance of Bayesian approaches. 
The implementations of Linear Logistic Regression, \mbox{$K$-Nearest Neighbours} and Linear SVM are based on~\cite{fan2008liblinear},~\cite{altman1992introduction} and~\cite{wu2007robust}, respectively. The Random Forest implementation is based on~\cite{breiman2001random}, whereas for the classifier based on Gaussian Processes we refer to~\cite{rasmussen2004gaussian}. Configuration parameters and implementation details for the benchmark classifiers are provided in Table~\ref{table_params}.

%We can therefore analyze the classification problems with a comprehensive perspective by comparing automatic feature extraction capabilities of deep NNs with other classifiers from the \mbox{state-of-the-art}.

\input{table_params}

%\subsubsection{Linear Classifiers}
%We focus on the linear logistic regression [REF] and linear \ac{SVM} [REF] as examples of linear classifiers. 
%%We consider as initial benchmarks, the so called Linear Classifiers. In particular, we focus on a linear \ac{SVM} and on the logistic regression. 
%%Both are discriminative models, that use the observed data $\bm{X}$, while learning the conditional probability $Prob(\bm{Y}|\bm{X})$ how to do the classification. Unlike generative models, which learn the joint probability $Prob(\bm{Y},\bm{X})$ they make fewer assumptions on the distribution of the data, but heavily depend on its quality.
%
%%Given a linear classifier, if the input feature vector is ${\bm{x}}$, then the output score  is:
%%\begin{equation}
%%\bm{y}=f({\bm{w}}\cdot {\bm {x}})=f\left(\sum _{j}w_{j}x_{j}\right)
%%\end{equation}	
%
%\medskip
%
%\textbf{Linear Logistic Regression} - Although it derives from linear regression, Linear Logistic Regression can be used to perform classification. In linear regression, the output  is modeled as a linear combination of features: $\bm{y} = \sum _{j}w_{j}x_{j} + b$. Differently, in the binary case, the logistic regression models the probability of the output as a linear combination of the features. The following is also called Logit function and defined as:
%\begin{equation}
%log\left(\frac{\pi}{1-\pi}\right) = \sum _{j}w_{j}x_{j}+b
%\end{equation}
%where $\pi$, in a binary case, is the probability of vector $\bm{x}$ to belong to one of the two class. It follows that $\pi$ is given by:
%\begin{equation}
%\pi = \frac{e^{\sum _{j}w_{j}x_{j} + b}}{1+e^{\sum _{j}w_{j}x_{j} + b}}=
%\frac{1}{1+e^{-{\sum _{j}w_{j}x_{j} + b}}},
%\end{equation}
%which is the Logistic function. For this reason, this classifier represents a particular case of a linear model, since it is the probability of belonging to a class that is modeled as a linear combination and not the actual output. In our problem, we adopt the implementation from the library presented in~\cite{fan2008liblinear}.
%
%\medskip
%
%\textbf{Linear SVM} - \ac{SVM} defines hyperplanes to separate the input data in the feature vector space and maximizes the margin around the separating hyperplane. The decision function is fully specified by the support vectors, a small subset of training samples.
%
%%In our problem, we use a linear SVM classifier to identify the different mobile apps. 
%In our implementation, we use the Hinge loss function~\cite{wu2007robust} to compute the \mbox{maximum-margin} classification. We use a standard L2-norm for regularization with the penalty parameter $C=0.025$. The library implementation details can be found here\cite{chang2011libsvm}.
%% For the loss, we use the Hinge loss function \angel{(Add ref here)} to compute the \mbox{maximum-margin} classification.
%%\begin{equation}
%%L(y)=\max(0,1-t\cdot y)
%%\end{equation}
%%where $y$ is the classifier score and $t\in \left(0,1\right)$ is the intended output.
%%Non-linear SVM can be implemented by applying a kernel function instead of the matrix multiplication, but the kernel selection and the analysis to obtain non linearities deserves a separate study.
%
%Both linear methods are originally intended for binary classification, but the extension from the binary case to a \mbox{multi-class} classification can be done using the \mbox{one-vs-all} scheme~\cite{fan2008liblinear}.
%
%\subsubsection{Random Forest} Random forest is an ensemble learning method [REF], which operates by constructing a multitude of decision trees at training time, and outputting the predicted class (i.e., service or app type in our case). With respect to larger decision trees, random forests are less prone to overfitting over the training dataset, since they are used to average multiple deep decision trees.
%
%Formally, the random forest consists of a collection of tree-structured classifiers $h(\bm{x_m},\theta_{n_t})$, where $n_t=1, ..., N_T$, $N_T$ is the number of trees, and $\theta_{n_t}$ are independent identically distributed random vectors, which account for the random choices we make when fitting the $n_t$-th tree~\cite{breiman2001random}. In our work, we choose $N_T=10$ and we use the bootstrap technique (also known as \textit{bagging}) for the random choices. 
%Being $\bm{x_m}$ the vector of the input sessions, $\bm{y_m}$ the output class, the bagging technique for random sampling is implemented according to the following pseudocode:
%
%\begin{algorithm}[h]
%	\caption{Bootstrap procedure for random forests.}
%	\SetAlCapSkip{2em}
%	\For{$n_t = 1 \dots N_T$}{
%		\For{$m = 1 \dots M$}
%		{
%			\begin{itemize}[leftmargin=*]{
%					\itemsep0.5em
%					\item sample with replacement
%					$\bm{x^m_{N_T}} <-\bm{x_m},
%					\bm{y}_{n_t} \bm{y_m}$\;
%					\item train the classification tree $h(\bm{x_m},\theta_{n_t})$ on  $X_{n_t}, \bm{y}_{n_t}$\;
%				}
%			\end{itemize}
%		}
%	}
%\end{algorithm}
%
%%Formally, the random forest consists of a collection of tree-structured classifiers $h(\bm{X},\theta_{n_t})$, where $n_t=1, ..., N_T$, $N_T$ is the number of trees, and $\theta_{n_t}$ are independent identically distributed random vectors, which account for the random choices we make when fitting the $n_t$-th tree~\cite{breiman2001random}. In our work, we choose $N_T=10$ and we use the bootstrap technique (also known as \textit{bagging}) for the random choices. 
%%Being $\bm{x}$ the vector of the input sessions, $\bm{y}$ the output class, the bagging technique for random sampling is implemented according to the following pseudocode:
%%Given $M$ the total number of sessions, $\bm{y}$ the output class vector and $N_T$ the total number of trees, the bagging technique for random sampling is implemented according to the following pseudocode:
%%\begin{algorithm}[h]
%%	\SetAlCapSkip{2em}
%%	\For{$n_t = 1 \dots N_T$}{
%%		{
%%			\begin{itemize}[leftmargin=*]{
%%					\itemsep0.5em
%%					\item sample, with replacement, $M$ training examples from $\bm{X}, \bm{y}$; these are $X_{n_t}, \bm{y}_{n_t}$\;
%%					\item train the classification tree $h(\bm{X},\theta_{n_t})$ on  $X_{n_t}, \bm{y}_{n_t}$\;
%%				}
%%			\end{itemize}
%%		}
%%	}
%%	\caption{Bootstrap procedure for random forests.}
%%\end{algorithm}
%
%\subsubsection{Gaussian Processes}
%%Bayesian \mbox{non-parametric} models, such as Gaussian Processes (GPs), can represent beliefs about the model parameters via a probability distribution (called the {\it prior} distribution). Then, Bayesian inference can reshape the prior distribution, transforming it into a {\it posterior} one. GPs have become popular for regression and classification, often showing impressive empirical performance.
%
%%A GP is a generalization of the Gaussian probability distribution and can be used for probabilistic classification. Formally, a GP is a collection of random variables, any finite number of which have a joint Gaussian distribution and it is completely specified by the mean function $m(x)$ and the covariance function $k(x, \hat x)$ .
%%\begin{equation}f(\cdot) \sim GP(m(x), k(x, \hat x))\end{equation}
%
%
%%For a binary classification task, we need to predict the probability $\pi(x)$, which lies in $[0,1]$:  the basic idea behind the Gaussian process prediction is to place a GP prior over the latent function $f(x)$ and then squash $f(x)$ through any sigmoid function to obtain a prior on $\pi(x) = \sigma(f(x))$. The latent function is a so-called nuisance function, whose values are not observed and are not relevant by themselves. Its purpose is to allow a convenient formulation of the model, and  is removed during prediction. Generally, the Logistic function is used to squash $f(x)$.
%
%%In contrast to a regression task, the posterior of the latent function $\pi(x)$ is not Gaussian even for a GP prior because of discrete class labels. Rather, a non-Gaussian likelihood corresponding to the logistic function is used. The approximation of the non-Gaussian posterior with a Gaussian likelihood is done by using the Laplace approximation. The details of the GP implementation can be found in~\cite{rasmussen2004gaussian}.
%
%Gaussian Processes (GPs) are a \mbox{non-parametric} approach to find a distribution over all the possible functions $f(x)$ that are consistent with the observed data. Similarly to other Bayesian methods, starts operation based on an initial distribution which is updated as data points are observed, producing the resulting distribution over functions.
%
%%Although to represent a distribution over a set of possible functions can be difficult, it turns out that only a distribution over the function's values at a finite, but arbitrary, set of points is needed.
%Formally, a GP is a collection of random variables, any finite number of which have a joint Gaussian distribution, and is completely specified by the mean $\mu(x)$ and covariance $\Sigma(x)$:
%\begin{equation}
%f(\cdot) \sim GP(\mu(x), \Sigma(x)).
%\end{equation}
%As described in~\cite{rasmussen2004gaussian}, GPs can be used for classification tasks, finding a probability $\pi(x)$ that lies in $[0,1]$. To this end, we need to define a prior Gaussian distribution over the latent function $f(x)$ and then squash $f(x)$ through any sigmoid function $\sigma$, to obtain a prior on $\pi(x) = \sigma(f(x))$.
%%The latent function is a \mbox{so-called} nuisance function, whose values are not observed and are not relevant by themselves. Its purpose is to allow a convenient formulation of the model, and is removed during prediction.
%In our work, the Logistic function is used to squash $f(x)$. The details of the GP implementation can be found in~\cite{rasmussen2004gaussian}.


==> Mobile Data Analysis - Journal/Conclusions.tex <==

\section{Conclusions}
\label{sec:conclusions}

In this paper, we have presented a framework that allows highly accurate classification of application and services from \mbox{radio-link} level data, at runtime, and without having to decrypt dedicated physical layer channels. To this end, we decoded the LTE Physical Downlink Control Channel (\ac{PDCCH}), where Downlink Control Information (\ac{DCI}) messages are sent in clear text. Through DCI data, it is possible to track the data flows exchanged between the serving cell and its active users, extracting features that allow the reliable identification of the apps/services that are being executed at the mobile terminals. For the classification of such traffic, we have tailored deep artificial Neural Networks \acp{NN}, namely, Multi-Layer Perceptron (MLP), Recurrent NNs and Convolutional NNs, comparing their performance against that of benchmark classifiers based on \mbox{state-of-the-art} supervised learning algorithms. Our numerical results show that NN architectures overcome the other approaches in terms of classification accuracy, with the best accuracy (as high as $98$\%) being achieved by \acp{CNN}. As a major contribution of this work, labeled and unlabeled datasets of DCI data from real radio cell deployments have been collected. The labeled dataset has been used to train and compare the classifiers. For the unlabeled dataset, we have augmented the \ac{CNN} with the capability of detecting input DCI data that do not conform to that learned during the training phase: the corresponding patterns are detected and associated with an {\it unknown} class. This increases the robustness of the \ac{CNN} classifier, allowing its use, at runtime, to perform fine grained traffic analysis from radio cell sites from an operative mobile network. To summarize, the main outcomes of our work are: \textbf{1)} a methodology to extract DCI data from the PDCCH channel, and for the use of such data to train traffic classifiers, \textbf{2)} the fine tuning and a thorough performance comparison of classification algorithms, \textbf{3)} the design of a novel technique for the {\it fine grained} and {\it online} traffic analysis of communication sessions from real radio cell sites, and \textbf{4)} the discussion of the traffic distribution resulting from such analysis from four selected sites of a Spanish mobile operator, in the city of Barcelona. 

%In this work we leverage on the \ac{LTE} \ac{PDCCH}, proposing a framework to collect and to classify the type of service and more specifically, the applications run by a certain user. In particular, we provided the following contributions: to the best of our knowledge, no \mbox{open-access} \mbox{\ac{PDCCH}-based} dataset is available in the literature, which can provide insightful information such as the actual base station scheduling, with a time resolution and granularity of $1$ms. Secondly, an exhaustive benchmarks is given, considering a wide-range class of algorithms: high accuracy ($> 97\%$) is obtained by the proposed architecture based on \ac{CNN}. Finally, a practical use-case is presented, by analyzing the dataset obtained during highly attended football matches, and we discuss about the benefits that can arise for the network planning and deployment from the use of the proposed framework. 


==> Mobile Data Analysis - Journal/Dataset.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=0.8\textwidth]{figures/framework_diagram5.png}
\caption{Experimental framework adopted for the creation of the unlabeled and labeled datasets. }
\label{fig:framework_diagram}
\end{figure*}

\section{Dataset Creation}
\label{sec:dataset}

Fig.~\ref{fig:framework_diagram} shows the different building blocks of the experimental framework that has been developed to populate the unlabeled and labeled datasets. Briefly, the {\it data measurement and collection} block acquires data from the LTE \ac{PDCCH} channel to extract the relevant \ac{DCI} information. {\it Data preparation}, instead, processes the gathered \ac{DCI} data so that it can be used for training and classification purposes.

\subsection{Data Collection System}

%Data collection embodies a relevant part in this work because of the exhaustive knowledge that we can gain about the network with it.
In LTE, the eNodeB communicates scheduling information to the connected \acp{UE} through the DCI messages that are carried within the PDCCH with a time granularity of $1$~ms. While the actual user content is sent over {\it encrypted dedicated channels}, i.e., the Physical Uplink/Downlink Shared Channel (PUSCH/PDSCH respectively), the \textbf{PDCCH is transmitted in clear text} and can be decoded. To process DCI data, we have adapted the OWL monitoring tool~\cite{bui2016owl}. A \ac{SDR} has been programmed, acquiring the \ac{PDCCH} via an \mbox{open-source} software sitting on top of the \mbox{srs-LTE} library~\cite{gomez2016srslte}, which makes it possible to synchronize and monitor the channel over a specified \ac{LTE} bandwidth. The SDR is connected to a PC that performs the actual decoding of DCI data: in our experimental settings, we used a low cost Nuand BladeRF x40 \ac{SDR} and an Intel \mbox{mini-NUC}, equipped with an i5 $2.7$~Ghz \mbox{multi-core} processor, $256$~GB \ac{SSD} storage and $18$~GB of RAM. 

\begin{figure*}[t]
	\centering
	\begin{subfigure}[t]{.49\columnwidth}
		\centering
		\includegraphics[width=\columnwidth]{figures/map_cttc.jpg}
		\caption{Castelldefels: suburban area with a university campus.\vspace{0.3cm}}
		\label{fig:castefa}
	\end{subfigure}
	%\quad
	\begin{subfigure}[t]{.49\columnwidth}
		\centering
		\includegraphics[width=\columnwidth]{figures/map_campnou.jpg}
		\caption{Camp Nou: mainly residential area with Barcelona FC stadium.\vspace{0.3cm}}
		\label{fig:bcn}	
	\end{subfigure}
	%\quad
	\begin{subfigure}[t]{.49\columnwidth}
		\centering
		\includegraphics[width=\columnwidth]{figures/map_paolo.jpg}
		\caption{Born: mixed residential, transport and leisure area.}
		\label{fig:born}	
	\end{subfigure}
	%\quad
	\begin{subfigure}[t]{.49\columnwidth}
		\centering
		\includegraphics[width=\columnwidth]{figures/map_marco.jpg}
		\caption{PobleSec: mainly residential area.}
		\label{fig:poblesec}	
	\end{subfigure}
	\centering
	\caption{Maps of Barcelona metropolitan areas where the measurement campaign took place for the creation of unlabeled and labeled datasets. In the maps, the \ac{eNodeB} location is denoted by $A$, whereas the data collection system and the mobile terminal are marked as B. In Castelldefels, the mobile terminal has been placed in two different locations (B$_1$ and B$_2$).}
	\label{fig:maps}
\end{figure*}


Decoded \ac{DCI} messages for a connected \ac{UE} contain the following scheduling information~\cite{etsi}:
\begin{itemize}
	\itemsep0.5em
	\item \ac{RNTI},
	\item \ac{RB} assignment,
	%Number of Allocated Resource Blocks (N\textsubscript{RB})
	\item \ac{MCS}.
	%\item \ac{TBS}
\end{itemize}


\ac{DCI} messages use \acp{RNTI} to specify their destination. \acp{RNTI} are \mbox{$16$-bit} identifiers that are employed to address \acp{UE} in an \ac{LTE} cell. They are used for different purposes such as to broadcast system information \mbox{(SI-RNTI)}, to page a specific UE \mbox{(P-RNTI)}, to carry out a random access procedure \mbox{(RA-RNTI)}, and to identify a connected user, i.e., the cell RNTI \mbox{(C-RNTI)}. In this work, we are interested in the \mbox{C-RNTI}, that is temporarily assigned when the UE is in RRC (Radio Resource Control) CONNECTED state, to uniquely identify it inside the cell. The \mbox{C-RNTI} can take any unreserved value in the range \mbox{[{\tt 0x003D}--{\tt FFF3}].} Once the \mbox{C-RNTI} is assigned to a connected \ac{UE}, the \ac{DCI} information directed to this terminal is sent using this \mbox{C-RNTI}, which is transmitted in clear text as part of the \ac{PDCCH} channel. Hence, knowing the \mbox{C-RNTI} allows tracking a specific connected user within the radio cell. Assuming that the \mbox{C-RNTI} is known (see Section~\ref{sec:labeled_dataset}), the following information about the ongoing communication for this \ac{UE} can be extracted from its \ac{DCI} data:

\begin{itemize}
\item {\it Number of allotted resource blocks:} in \ac{LTE}, a \ac{RB} represents the smallest resource unit that can be allocated to any user. The number of resource blocks that are assigned to a \ac{UE} (N\textsubscript{RB}), is derived based on the \ac{DCI} bitmap.

\item {\it Modulation order and code rate:} the \ac{MCS} is a \mbox{$5$-bit} field that determines the modulation order and the code rate that are used, at the physical layer, for the transmission of data to the UE.

\item {\it \ac{TBS}:} the \ac{TBS} specifies the length of the packet to be sent to the \ac{UE} in the current \ac{TTI}. It is derived by from a lookup table by using \ac{MCS} and N\textsubscript{RB}, see~\cite{etsi}.
\end{itemize}
In this work, we demonstrate that monitoring the downlink and uplink \ac{TBS} information of a given \ac{UE} enables service and app classification with high accuracy.

\subsection{Unlabeled Dataset}
\label{sec:unlabeled_dataset}

Thanks to the just described \ac{DCI} collection system, four cell sites of a Spanish mobile network operator in the metropolitan area of Barcelona have been monitored for a full month. The selected \acp{eNodeB} are located in areas having different demographic characteristics and land uses, so as to diversify the captured traffic in terms of service and app behavior. We have named the datasets according to the corresponding neighborhood: {\it PobleSec} (mainly residential area), {\it Born} (mixed residential, transport and leisure area), {\it Castelldefels} (mixed suburban and campus area), {\it Camp Nou} (mixed residential and stadium area). In total, we have collected more than $68$~GB of \ac{DCI} data from the \ac{LTE} \ac{PDCCH}. Fig.~\ref{fig:maps} shows the locations of the four monitored sites, along with that of the data collection system. After the data collection, the signaling associated with each active \mbox{C-RNTI} is extracted from the \ac{PDCCH} \ac{DCI} data stream, and is prepared for the classifier. During this, we discarded \mbox{short-length} traces, which are mainly due to signaling, paging and background traffic. These accounted for less than $3\%$ of the total traffic in the monitored radio cells.

\subsection{Labeled Dataset}
\label{sec:labeled_dataset}

A {\it labeled} dataset is obtained by running specific services and apps at a mobile terminal under our control, detecting its \mbox{C-RNTI} within the \ac{PDCCH} channel and finally associating the corresponding \ac{DCI} trace with a {\it label}, which links it to the service/app that is executed at the \ac{UE}. Generating data sessions is easy, and boils down to running a specific app from a device that we control, and that is connected to the monitored \ac{eNodeB}. The difficult part is to identify the generated data flow among those carried by the \ac{PDCCH} channel, which contains \ac{DCI} information for {\it all} the connected \acp{UE} within the radio cell. We made this labeling possible by injecting a {\it watermark} into the traffic that we generated by the controlled \ac{UE}, so that it could be easily identified among all other users.

\subsubsection{Data preparation and watermarking} The data preparation procedure is divided into two phases: \textbf{1)} the {\it identification} of the \mbox{C-RNTI} corresponding to the controlled \ac{UE}, \textbf{2)} the {\it extraction} and {\it labeling} of the corresponding \ac{DCI} trace. In the \ac{LTE} \ac{PDCCH} channel, each \ac{UE} is identified by the \mbox{C-RNTI}, which uniquely identifies the mobile terminal within the radio cell. This identifier is {\it temporary}, i.e., it changes after short inactivity periods. This is done to prevent the plain tracking of mobile users, since the \ac{PDCCH} is sent unencrypted. To allow traffic labeling (i.e., user identification), we introduced a {\it watermark} into the traffic generated through our mobile terminal. This watermark amounts to producing, for each application, a regular pattern: any given application (e.g., YouTube) is run for a \mbox{pre-defined} amount of time ($60$~seconds in our measurements), then, a pause interval of fixed duration is inserted before running the app for further $60$~seconds. We loop this over time, obtaining a duty cycled activity pattern that is easily distinguishable from all the other activity traces within the radio cell. Through this watermarking procedure, we could successfully associate our \ac{UE} with the corresponding \mbox{C-RNTI} from the \ac{DCI}. Also, we split the traces into different sessions thanks to the duty cycled pattern, where subsequent sessions are separated by the pause interval (of fixed duration). The {\it label}, corresponding to the application that is being executed at the mobile terminal, was finally associated with the extracted \ac{DCI} data.


In our measurement campaign, we have recorded and labeled about $M=10,000$ mobile sessions, gathering the scheduling information contained in the \ac{DCI} messages for selected apps. We considered three \mbox{data-intensive} services: {\it video streaming}, {\it audio streaming} and {\it \mbox{real-time} video calling}, which represent classes producing a considerable amount of traffic and taking most of the network resources~\cite{ericsson}. For each service type, we chose two popular applications: \textit{Spotify} and \textit{Google Music} for audio, \textit{YouTube} and \textit{Vimeo} for video streaming, while for the video calling we picked two \mbox{instant-messaging} applications, namely, \textit{Skype} and \textit{WhatsApp Messenger}.



A large measurement campaign was conducted to expose the mobile terminal running the selected apps to different {\it radio link conditions}, thus obtaining a comprehensive dataset. In particular, the \ac{UE} was placed into two different locations (termed B$_1$ and B$_2$ in Fig.~\ref{fig:castefa}) within the Castelldefels radio cell to experience different received signal qualities ($-84$~dBm and $-94$~dBm for B$_1$ and B$_2$, respectively), and in the Camp Nou \ac{eNodeB} during football matches, to capture data in high cell load conditions.

\begin{figure*}[t]
	\centering
	\includegraphics[width=2\columnwidth]{figures/trace_vs_time}
		\includegraphics[height=4.2cm]{figures/video_vs_time_uplink}
	\includegraphics[height=4.2cm]{figures/audio_vs_time_uplink}
	\includegraphics[height=4.2cm]{figures/call_vs_time_uplink}
	\caption{Traffic pattern snapshots showing the normalized data rate for different applications as a function of time.}
	\label{fig:trace_vs_time}
\end{figure*}

Fig.~\ref{fig:trace_vs_time} shows a few radio resource usage patterns collected for the selected apps. Some similarities can be recognized within the same service class. For example, audio and video streaming present similar behaviors. Also, significant differences can be observed between the radio resource usage of real time video calls (\textit{Skype} and \textit{WhatApp Video}) and the other apps. Video and audio streaming applications use up a high amount of radio resources at the beginning of the sessions, buffering most of the content into the terminal memory. Real time video calling, instead, entails a continuous transmission and a more constant usage of radio resources throughout the sessions. Note that the amount of data exchanged in the uplink direction is significant only for this service class, since a video call requires a bidirectional communication.

\subsection{Synchronous and Asynchronous Sessions}

Through the watermarking approach and the splitting procedure, we obtained a labeled dataset, where each session, depending on the service, presents patterns similar to those shown in Fig.~\ref{fig:trace_vs_time}. Assuming that the beginning and the end of each session are known is rather optimistic, as in a real measurement setup we have no means to accurately track these instants. Put it another way, it is unlikely that the LTE PDCCH measurements and the application run on the \ac{UE} will be temporally \textit{synchronized}. Synchronizing the measurement with the beginning of each session would facilitate the classification task, since most of the generated traffic is buffered on the terminal at the beginning, see Fig.~\ref{fig:trace_vs_time}, and this behavior is a distinctive feature that is easy to discriminate. %across services and apps.

To ensure the applicability of our classifiers to real world (asynchronous) cases, we account for \textit{asynchronous} sessions, entailing that the classification algorithm has no knowledge about the instants where the sessions begin and end. Specifically, each session is split using a sliding window of length $W$~seconds, moved rightwards from the beginning of the session with a stride of $S$~seconds, see Fig.~\ref{fig:slide_win}. The split sessions (asynchronous sessions), of $W$ seconds each, represent the input data to our classification algorithms. Note that $W$ and $S$ are \mbox{hyper-parameters} of the proposed classification frameworks. 

\begin{figure}[t!]
	\centering
	\includegraphics[width=.9\columnwidth]
	{figures/slide_win}
	\caption{Sliding window of $20$s length and $15$s stride, applied to a sample \mbox{video-streaming} session.}
	\label{fig:slide_win}
\end{figure}

\subsection{Sessions Correlation over Time}

As a sanity check, we verify the soundness of the watermarking strategy: our aim is to understand whether the transmission of user data in the form of duty-cycled patterns may affect the way in which the eNodeB handles the communication from our terminal, e.g., through some advanced channel reservation mechanism. In that case, in fact, our watermarking strategy would be of little use, as it would introduce scheduling artifacts that do not occur in real life conditions. To verify this, we evaluated the Pearson correlation between the initial session (i.e., when the \ac{UE} connects to the LTE PDCCH for the first time and it is assigned a new \mbox{C-\ac{RNTI}}) and the following ones. Fig.~\ref{fig:correlation} shows that, for each of the three services, the correlation is high only when we compare the first session with itself ($n=0$). Instead, low values are observed between the first session and the following ones ($n>1$), indicating that the behavior of the eNodeB scheduler is not affected by the repetitive actions (i.e., the \mbox{duty-cycled} activity) performed at the \ac{UE} side. 

\begin{figure}[t!]
	\centering
	\includegraphics[width=.9\columnwidth]
	{figures/correlation}
	\caption{
	Pearson correlation between the initial and the following sessions running in the controlled UE.
	}
	\label{fig:correlation}
\end{figure}

==> Mobile Data Analysis - Journal/Introduction.tex <==
\section{Introduction}
\label{sec:intro}


%\IEEEPARstart{W}{ith} the advent of powerful chipsets, \mbox{high-definition} \mbox{bezel-less} screens, and upgraded memory storages, mobile devices have become information and communication hubs and are getting more powerful by the day. Starting with 4G, mobile applications (apps) are as well getting resource hungry, requiring large bandwidth and good amount of computation at the devices. The demand for streaming application is increasing at a constant pace, for example, more than half of YouTube views come from mobile terminals~\cite{ericsson,ciscovni}, and future networks are called to be highly responsive in any context, e.g., \mbox{high-speed} mobility, indoor, crowded events, etc.~\cite{chen2014requirements}.

%Starting from 4G, mobile networks must comply with the pressing requirements dictated by resource heavy \acp{app}, such as gaming, video streaming, etc., which require a large bandwidth and, often, low latencies. Videos already constitute the largest majority of content available online, and more than half of YouTube views come from mobile devices~\cite{ericsson},\cite{ciscovni}. Thus, mobile networks represent an opportunity to deliver an ever growing number of ubiquitous multimedia applications. 
%Bearing these facts in mind, mobile technology is being challenged to keep the pace of hardware and application advancements. To satisfy the uprising demand from mobile users, 5G (and beyond) networks are called to be highly responsive in any context, e.g., \mbox{high-speed} mobility, indoor, crowded events, etc.~\cite{chen2014requirements}.
%A key feature towards supporting such technological evolution, and the corresponding upsurge in multimedia traffic, is represented by the ability of networks to carry out automatic traffic analysis, through {\it online classification tools}. The categorization of network traffic into appropriate classes has many relevant uses spanning from Quality of service (QoS)/Quality of Experience (QoE) control and management, to pricing, network resource management, malware detection, and intrusion detection, to name a few. 

\IEEEPARstart{W}{ireless} mobile technology is advancing at a fast pace, through better monitor resolutions, larger memories, higher communication speeds, etc., and, with that, more requirements in terms of supported data rates~\cite{ericsson,ciscovni}, new services, and a higher network responsiveness across diverse physical contexts~\cite{chen2014requirements}.

In this work, we design and evaluate, via a \mbox{proof-of-concept} implementation, \mbox{non-intrusive} tools for the online estimation of \ac{LTE} cellular activity, i.e., the type of traffic that users exchange with their serving base station. As we quantify, our technology allows one to infer {\it with high accuracy} the service (e.g., audio, video, etc.) and the application (e.g., Skype, Vimeo, You Tube, etc.) that are being used by the connected mobile users. This is accomplished by decoding LTE downlink/uplink control channel messages (i.e., \mbox{radio-link} level data), which are transmitted in clear text and without breaking any security protocol (encryption). We believe that this brings a high value along several dimensions:
\begin{itemize}
\item first, our tool permits a better understanding of spectrum needs across time and space. Note that there are limited means to \mbox{non-intrusively} monitor user density and traffic demand in \mbox{real-time}. These measurements are key for the correct dimensioning of future mobile systems, and the investigation of new data communication and processing techniques at the network edge. In fact, although network operators gather such data through their base stations, they seldom release it due to privacy concerns, so these measures are almost never used for research purposes by university, public or private research labs. We only found a limited number of datasets available including mobile data traffic~\cite{Laurila2012}\cite{Barlacchi2015}, but they are often incomplete, poorly documented and contain aggregated data, often averaged hourly or across a certain geographic area. Our technique allows the extraction of data flows with a granularity of one second, isolating the amount of data, the type of service and application exploited by each mobile user within an LTE cell. We believe that this has a high value for researchers within the mobile networking space, who will be able to create their own {\it rich} datasets for research purposes, to spur the advancement of future edge communication (and computing) technology; 
\item second, our work sheds new light on possible attacks that may be carried out by exploiting the LTE control channel data. In fact, being able to track user density across time and space by just deploying a number of sniffers within a city may be also exploited maliciously, for example to infer details about mobility and user density. While such analysis, so far, has been carried out with data from network operators, e.g., the Telecom Italia mobile challenge~\cite{Reades2009}, our tool allows the extraction of fine grained LTE data in full autonomy. This may represent a privacy concern.  
\end{itemize}

A large body of work exists in the area of mobile traffic classification (see Section~\ref{sec:related} for an in depth discussion of the related work). The key challenge of existing classification algorithms consists in the identification, and in the subsequent computation, of a number of {\it representative features}. These features are then used to train algorithms that classify the data flows at runtime. Most of the surveyed approaches leverage some {\it domain knowledge}, which is utilized to {\it manually} obtain the feature set, i.e., by a skilled human expert. However, the use of deep learning techniques has recently paved the way to automatic feature discovery and extraction, often leading to superior performance. For example, in~\cite{aceto2018mobile} encrypted traffic is categorized through deep learning architectures, proving their superior performance with respect to shallow neural network classifiers. The authors of~\cite{zhang2017zipnet} present a mobile traffic \mbox{super-resolution} technique to infer narrowly localized traffic consumption from coarse measurements: a \mbox{deep-learning} architecture combining Zipper Network (ZipNet) and Generative Adversarial neural Network (GAN) models is proposed to accurately reconstruct \mbox{spatio-temporal} traffic dynamics from measurements taken at low resolution. In~\cite{chen2016automatic}, the identification of mobile apps is carried out by automatically extracting features from labeled packets through \acp{CNN}, which are trained using raw \ac{HTTP} requests, achieving a high classification accuracy. We stress that the work in these papers, as the majority of the other techniques discussed in Section~\ref{sec:related}, use statistical features obtained from application or \mbox{\ac{IP}} level information for both service and app identification, along with UDP/TCP port numbers.

The solution here presented sharply departs from previous approaches, as it performs highly accurate traffic classification directly from {\it radio-link} level data, without requiring any prior knowledge and without having to decode and/or decrypt the transmitted data flows. The proposed classifiers enable fully automated, over the air, and detailed traffic profiling in mobile cellular systems, making it possible to infer, in an online fashion, the radio resource usage of typical service classes. To do this, we leverage OWL~\cite{bui2016owl}, a tool that allows decoding the \ac{LTE} \ac{PDCCH}, where control information is exchanged between the \ac{LTE} \ac{eNodeB} and the connected \acp{UE}. Specifically, we decode the \ac{DCI} messages carried in the \ac{PDCCH}, which contain \mbox{radio-link} level settings for the user communication (e.g., modulation and coding scheme, transport block size, allocated resource blocks). From \ac{DCI} data, we create two datasets
\begin{itemize}
\item[\textbf{1)}] a \emph{labeled dataset}, used to {\it train} service and app classification algorithms, where labeling is made possible by injecting an easily identifiable watermark into the application flows generated by a  terminal under our control; 
\item[\textbf{2)}] an \emph{unlabeled dataset}, used for {\it traffic profiling} purposes, which is populated by monitoring, for a full month, mobile traffic from four operative radio cell sites with different demographic characteristics within the metropolitan area of Barcelona, in Spain.
\end{itemize}

For the traffic analysis, we focus on a few services and applications that dominate the radio resource usage, but the approach can be readily extended to further services and applications. We directly use raw DCI data as input into deep learning classifiers (automatic feature extraction), achieving accuracies as high as $98$\% for both mobile service and app identification tasks. Moreover, we propose a novel technique to use our best classifier in {\it unsupervised settings}, to profile the mobile traffic from operative radio cell sites at runtime. Our tool allows for a {\it fine grained} and {\it automated} analysis of user traffic from real deployments, using radio link messages transmitted over the \ac{PDCCH}. The developed classification algorithms, as well as our experimental results are highly novel within the traffic monitoring literature, which only provides hourly and {\it aggregated} measures for typical days~\cite{earth-D23}\cite{Xu2017understanding}, and where traffic profiling is performed from UDP/TCP, IP or above IP flows, e.g.,~\cite{aceto2018mobile, zhang2017zipnet, chen2016automatic}.

In summary, the original contributions of this work are

\begin{itemize}
	\item \textit{Mobile Data Labeling:} we present an original and effective approach to automatically label \ac{LTE} PDCCH \ac{DCI} data traces. This approach is utilized for six mobile apps, to create a unique correspondence between the software programs (the apps) and the session identifiers that were assigned to them by the eNodeB. The result is a {\it labeled dataset} of real \ac{DCI} data from selected applications, i.e., YouTube, Vimeo, Spotify, Google Music, Skype and WhatsApp video calls.
	\item \textit{Classification and Benchmarks:} we tailor deep artificial Neural Networks (NNs), namely \mbox{Multi-Layer} Perceptron (MLP), \acp{RNN} and \acp{CNN}, to perform classification tasks for mobile services and app identification on the labeled dataset. Moreover, we compare their performance against a number of (benchmark) \mbox{state-of-the-art} classifiers. %\ac{CNN} architectures achieve the highest classification accuracy.
	\item \textit{Mobile Data Collection from an Operative Mobile Network:} we collect real \ac{LTE} PDCCH \ac{DCI} data traces, with a time granularity of $1$~ms, from four \acp{eNodeB} located in the metropolitan area of Barcelona, in Spain. Each of these datasets has a duration of $1$~month.
	\item \textit{Mobile Service Profiling from Unlabeled Data:} the \ac{CNN} classifier, which is found to be the best among all \ac{NN} schemes, is augmented with the capability of rejecting {\it out of distribution} sessions, i.e., sessions whose statistical behavior departs from those learned during the training phase. This makes it possible to use it with unlabeled traffic (online and unsupervised settings). The augmented \ac{CNN} classifier rejects those sessions for which it is uncertain, providing a robust classification outcome. Through its use, the four selected \acp{eNodeB} are monitored, getting a fine grained traffic decomposition. %The proposed augmentation strategy exploits theoretically sound and lightweight techniques, and constitutes an innovative contribution of this paper.
	%Our results are successfully \mbox{cross-validate} against those of other profiling studies form the literature, based on data of different nature, and obtained through different methodologies.
\end{itemize}

The paper is organized as follows. Section~\ref{sec:dataset} presents the experimental framework and the proposed methodology to obtain the two datasets. Section~\ref{sec:sl} introduces the two classification problems, namely, service and app identification and presents the classification algorithms. The performance of such classification algorithms is assessed in Section~\ref{sec:results}. In Section~\ref{sec:traffic_profilig}, the \ac{CNN} classifier is augmented with the capability of rejecting out of distribution sessions. Thus, the mobile traffic from four selected cell sites of an operative mobile network in Spain is decomposed over a full day. The related work on mobile traffic classification is reviewed in Section~\ref{sec:related}, and some concluding remarks are provided in Section~\ref{sec:conclusions}.



==> Mobile Data Analysis - Journal/Neural_Networks.tex <==
%!TEX root = main.tex

\section{Neural Networks}
\label{sec:nn}

In this section, we present three approaches based on neural networks used for the traffic classification problem. Specifically, we have employed a \ac{MLP}, a \ac{RNN} network and a \ac{CNN}. Details about the customized architectures are provided hereafter. It should be noted that the layer settings provided for each \ac{NN} are specific for the obtained dataset explained in Section~\ref{sec:dataset}, with the goal of obtaining the highest performance in terms of accuracy, with the lowest complexity. In contrast to previous methods presented in Section~\ref{sec:sl}, these tools enable automatic feature detection within the raw dataset traces, which provides an improvement in the classification performance as we will show shortly in Section~\ref{sec:results}.

\subsection{Multilayer Perceptron}
\label{sec:nn_mlp}
A multilayer perceptron is a \mbox{feed-forward} (the input signal goes only one way within the network) artificial neural network  that generates a set of outputs from a set of inputs. An MLP is characterized by, at least, three layers of nodes: an input, a hidden layer and an output, and these layers are connected as a directed graph between the input and output layers. Except for the input nodes, each node is a neuron that uses a nonlinear activation function to produce an output. MLP utilizes a supervised learning technique called backpropagation for training, i.e., to find the weights for each neuron within the network that minimize a certain error objective function. It can distinguish data that is not linearly separable. For further details, please refer to \cite{bishop2006}.

In the present work, the customized \ac{MLP} architecture we have used for the classification is composed by three fully connected layers. Details are as follows. First, an input layer ${MLP}_1$ with $N_{{MLP}_1}= 128$ neurons is used, where each neuron uses a leaky version of a \ac{ReLU}. The ReLU activation function is used a lot in neural network architectures and allows the activation to be thresholded at zero. However, during the training, large gradient flows through a ReLU neuron can cause the weights to update in such a way that the neuron will never activate on any data point again. If this happens, then the gradient flowing through the unit will forever be zero from that point on, and the neuron will be useless. Leaky \acp{ReLU} attempt to solve this, by forcing the function to have a small negative slope rather than zero value. The leaky \ac{ReLU} activation function has been used due to the need of tackling \mbox{non-linearities} present in the dataset. Given an input $x$, it is defined as follows:
%
\begin{equation}
	f(x) = \left\{ 	\begin{array}{lr} 	\alpha x & : x < 0\\ 	x & : x \ge 0 	\end{array} \right.
\end{equation}

\noindent where $\alpha$ controls the negative slope and usually takes values around $0.1$.
Moreover, the use of only linear activation functions in every layer would imply that the final activation function of the last layer would be just a linear function of the first layer input. This means that several layers can be replaced by a single layer, losing the ability of stacking layers and its improvement in finding hidden features within the input dataset.
Then, there is a second fully connected layer ${MLP}_2$, i.e., each output neuron is connected to all input neurons of this layer (weights are not shared), that comprises $N_{{MLP}_2}= 64$ neurons with the same activation function as the first one. Finally, each output neuron in the last layer ${MLP}_3$ corresponds to a specific class $k \in K$, where $K=6$ classes for app classification and $K=3$ for service classification. 

The output vectors of all layers have binary entries and are \mbox{hot-encoded}, i.e., all values are zero except for the entry corresponding to the output chosen class. The output of layer ${MLP}_3$ is a stochastic vector $\bm{y}$ obtained by a softmax activation function, whose $k$-th entry $k = 1,2,\dots,K$ can be seen as the probability that the input pattern belongs to class $k$, i.e., $y_k = y_k(\bm{w},\bm{X}) = Prob(t_k = 1|\bm{w},\bm{X})$, where $\bm{w}$ is the vector containing all the \ac{MLP} weights, $\bm{X}$ is the current input matrix and $t_k = 1$ if $\bm{X}$ belongs to class $k$ and $t_k = 0$ otherwise. If $\bm{X}$ is the set of all training examples, we define the batch set as $\mathcal{B} \subset \mathcal{X}$. Let $\bm{X} \in \bm{B}$ and denote the corresponding output vector by $\bm{y}(\bm{w},\bm{X})$ and its $k$-th entry by $y_k(\bm{w},\bm{X})$. The corresponding target vector is $\bm{t(X)} = (t_1(\bm{X}), \dots, t_k(\bm{X}))^T$ \cite{gadaleta2016idnet}. The network is trained in a supervised manner solving a \mbox{multi-class} classification problem using the {\it RMSprop} algorithm~\cite{tieleman2012lecture}, a specific gradient descend algorithm which minimizes a categorical \mbox{cross-entropy} loss function $L(\bm{w})$, defined as \cite{bishop2006} (Eq. (5.24) of Section 5.2):

\begin{equation}
\label{eq:cross}
	L(\bm{w}) = - \sum_{\bm{X} \in \bm{B}} \sum_{k=1}^{K} t_k(\bm{X}) log(y_k(\bm{w},\bm{X})).
\end{equation}

During training, Eq.~\ref{eq:cross} is iteratively minimized, by rotating training examples in the batch set $\mathcal{B}$ so as to span the entire input set $\mathcal{X}$. 

\subsection{Recurrent Neural Network}
\label{sec:nn_rnn}
\ac{RNN} are a generalization of feedforward neural networks, that have been devised for handling temporal and predictive problems. \ac{LSTM} networks are a particular kind of \ac{RNN}, introduced in \cite{Hochreiter1997}. They have been explicitly designed to avoid the \mbox{long-term} dependency issue, which is the cause of the \mbox{vanishing-gradient} problem in normal \acp{RNN} \cite{gers1999learning}.

The capability of learning \mbox{long-term} dependencies is due to the structure of the \ac{LSTM} units, which incorporates gates that regulate the learning process. The neurons in the hidden layers of an \ac{LSTM} are \acp{MC}. A \ac{MC} has the ability to store or forget information about past network states by using structures called {\it gates}, which consist of a cascade of a neuron with sigmoidal activation function and a pointwise multiplication block. Thanks to this architecture, the output of each memory cell possibly depends on the entire sequence of past states, making \acp{LSTM} suitable for processing time series with long time dependencies~\cite{Hochreiter1997}. An \ac{LSTM} memory cell diagram is presented in Fig.~\ref{fig:lstm_diagram}. The input gate is a neuron with sigmoidal activation function ($\sigma$). Its output determines the fraction of the MC input that is fed to the cell state block. Similarly, the forget gate processes the information that is recurrently fed back into the cell state block. The output gate, instead, determines the fraction of the cell state output that is to be used as output of the MC at each time step. Gate neurons usually have sigmoidal activation functions ($\sigma$), while the input and cell state use the hyperbolic tangent ($\tanh$) activation function. All the internal connections of the \ac{MC} have unitary weight~\cite{Hochreiter1997}.

\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{figures/lstm_cell.eps}
	\caption{\ac{LSTM} memory cell diagram.}
	\label{fig:lstm_diagram}
\end{figure} 

\begin{figure}[t]	
	\centering
	\includegraphics[width=\columnwidth]{figures/lstm.eps}
	\caption{\ac{RNN} architecture.}
	\label{fig:lstm_nn}	
\end{figure}

The proposed architecture for the traffic classification is depicted in Fig.~\ref{fig:lstm_nn}. In our design, we consider three stacked layers combining two LSTM layers with a final output fully connected layer. The first layer ${RNN}_1$ is composed by $N_{{RNN}_1}= 180$ \acp{MC} and the second one ${RNN}_2$ has $N_{{RNN}_2}= 180$ as well. The final fully connected layer ${RNN}_3$ performs the actual \mbox{multi-class} classification as the final layer in the \ac{MLP} network. Hence, the explanation given in \ref{sec:nn_mlp} about it also applies here. Moroever, the same optimizer to minimize Eq.~\ref{eq:cross} has been used in this case.

\subsection{Convolutional Neural Network}
\label{sec:nn_cnn}

\acp{CNN} are \mbox{feed-forward} deep neural networks differing from fully connected multilayer networks for the presence of one or more convolutional layers. At each convolutional layer, a number of kernels is defined. Each of them has a number of weights, which are convolved with the input in a way that the same set of weights, i.e., the same kernel, is applied to all the input data, moving the convolution operation across the input span. Note that, as the same weights are reused (shared weights), and each kernel operates on a small portion of the input signal, it follows that the network connectivity structure is sparse. This leads to advantages such as a considerably reduced computational complexity with respect to fully connected feed forward neural
networks \cite{gadaleta2016idnet}. For more details the reader is referred to \cite{goodfellow2016deep}. CNNs have been proven to be excellent feature extractors for images \cite{gadaleta2016idnet} and here we prove their effectiveness for mobile traffic data. 

The \ac{CNN} architecture that we designed to this purpose is shown in Fig.~\ref{fig:cnn}. It is composed of a cascade of two convolutional layers, followed by a pooling layer respectively, and finally a  \mbox{two-layer} fully connected network. The convolutional layers in combination with the first fully connected layer perform a dimensionality reduction (or automatic feature extraction) task, whereas the last fully connected one performs the \mbox{multi-class} classification. The first convolutional layer $CNN_1$ uses one dimensional kernels ($1$x$5$ samples) performing a first filtering of the input and processing each input vector (rows of $\bm{X}$) separately. The activation functions are linear and the number of convolutional kernels is referred to as $N_{{CNN}_1}=32$. 
The second convolutional layer $CNN_2$ uses again one dimensional kernels ($1x5$ samples) with  non-linear hyperbolic tangents as activation functions, and the number of convolutional kernels is referred to as $N_{{CNN}_2}=64$.
Max pooling is applied to the output of $CNN_1$ and $CNN_2$ to further reduce its dimensionality and increase the spatial invariance of features \cite{gadaleta2016idnet}. In both cases, a \mbox{one-dimensional} pooling with kernel $1$x$3$ is performed. Finally, th fully connected network is composed of two layers. The first one $CNN_3$ helps in finding hidden features from the input data and has $N_{{CNN}_2}=32$ neurons with leaky \ac{ReLU} activation function. It has been added to reduce computation time while achieving the same accuracy as compared with the case where a third convolutional layer was added. The final output layer $CNN_4$ follows the same architecture as previously mentioned (see last paragraph of Section~\ref{sec:nn_mlp}).

\begin{figure}[t]	
	\centering
	\includegraphics[width=\columnwidth]{figures/cnn.eps}
	\caption{\ac{CNN} architecture.}
	\label{fig:cnn}	
\end{figure}


==> Mobile Data Analysis - Journal/Related_Work.tex <==

\section{Related Work}
\label{sec:related}

The most common classification methods in the literature leverage UDP/TCP port analysis and/or packet inspection. 

UDP/TCP port analysis relies on the fact that most Internet applications use \mbox{well-known} \ac{TCP} or \ac{UDP} port numbers. For instance, the authors of~\cite{choi2012automated} define a mobile traffic classifier as a collection of rules, including destination \ac{IP} addresses and port numbers. Based on these rules, \mbox{application-level} mobile traffic identification is performed deploying a dedicated classification architecture within the network, and measurement agents at the mobile devices. However, \mbox{port-based} schemes hardly work in the presence of applications using dynamic port numbers~\cite{fu2016service}. 

A scheme based on deep packet inspection is presented in~\cite{yang2012empirical}. The authors of this paper devise a technique for \ac{CDMA} traffic classification, using \mbox{correlation-based} feature selection along with a decision tree classifier trained on a  labeled dataset (which is labeled via deep packet inspection). The algorithm in~\cite{han2012maximum} extracts application layer payload patterns, and performs maximum \mbox{entropy-based} \mbox{IP-traffic} classification exploiting different \ac{ML} algorithms such as Naive Bayes, \acp{SVM} and partial decision trees. Remarkably, \mbox{payload-based} methods are limited by a significant complexity and computation load~\cite{fu2016service}. Furthermore, many mobile applications adopt encrypted data transmission due to security and privacy concerns, which renders packet inspection approaches ineffective. 

Classification schemes for encrypted flows utilize traffic statistics, extracting meaningful features from the observed traffic patterns. For example, the authors of~\cite{liu2018cascade} propose a classification system for mobile apps based on a Cascade Forest algorithm exploiting features related to: i) the mobile traces, ii) the Cascade Forest algorithm, iii) \mbox{connection-oriented} protocols and \mbox{connection-less} protocols, and iv) encrypted and \mbox{unencrypted} flows. Along the same lines, a classification approach that combines \mbox{state-of-art} classifiers for encrypted traffic analysis is put forward in~\cite{aceto2018mobile}.

Another interesting work is presented in~\cite{fu2016service}, where the authors classify service usage from mobile messaging apps by jointly modeling user behavioral patterns, network traffic characteristics, and temporal dependencies. The framework is built upon four main blocks: traffic segmentation, traffic feature extraction, service usage prediction, and outlier detection. When traffic flows are short and the defined features do not suffice to fully describe the traffic pattern, \acp{HMM} are exploited to capture temporal dependencies, to enhance the classification accuracy.

The authors of~\cite{2016eavesdropping} show that a passive eavesdropper is capable of identifying fine grained user activities for \mbox{Android} and iOS mobile apps, by solely inspecting \ac{IP} headers. Their technique is based on the intuition that the highly specific implementation of an app may leave a fingerprint on the generated traffic in terms of, e.g., transfer rates, packet exchanges, and data movement. For each activity type, a behavioral model is built, then \mbox{K-means} and \ac{SVM} are respectively used to reveal which model is the most appropriate, and to classify the mobile apps. 

Automatic fingerprinting and \mbox{real-time} identification of Android apps from their encrypted network traffic is presented in~\cite{taylor2016appscanner}. \mbox{IP-based} feature extraction and supervised learning algorithms are the basis of a framework featuring six classifiers, obtained as variations of \acp{SVM} and \acp{RF}. \acp{RF} have also been considered in~\cite{2015enhancing}, where the authors claim that the sole use of \mbox{packet-based} features does not suffice to classify the traffic generated by mobile apps. As a solution, they  use a combination of packet size distributions and communication patterns. 

Recent works exploit \acp{NN}~\cite{chen2016automatic}\cite{zhang2017zipnet}\cite{aceto2018mobile}. In~\cite{chen2016automatic}, mobile apps are identified by automatically extracting features from labeled packets through \acp{CNN}, which are trained using raw \ac{HTTP} requests. In~\cite{aceto2018mobile}, encrypted traffic is classified using deep learning architectures (feed forward, convolutional and recurrent neural networks) for \mbox{Android} and iOS mobile apps, with and without using TCP/UDP ports. The authors of~\cite{zhang2017zipnet} combine Zipper Networks (ZipNet) and \ac{GAN} to infer narrowly localized and fine grained traffic generation from coarse measurements.

A systematic framework is devised in~\cite{aceto2019mobile} for comparison among different techniques where deep learning is proposed as the most viable strategy. The performance of the deep learning classifiers is thoroughly investigated based on three mobile datasets of real human users’ activity, highlighting the related drawbacks, design guidelines, and challenges.
%
Several survey papers dealing with deep learning techniques applied to traffic classification can be found in~\cite{rezaei2019deep}, ~\cite{wang2019survey} and~\cite{zhang2019deep}. The authors in~\cite{rezaei2019deep} overview general guidelines for classification tasks, present some deep learning techniques and how they have been applied for traffic classification, and finally, open problems and future directions are addressed. 
%
The survey in~\cite{wang2019survey} presents a deep learning-based framework for mobile encrypted traffic classification, reviewing existing work according to dataset selection, model input design, and model architecture, and highlighting open issues and challenges.
%
Finally, a comprehensive and thorough study of the crossovers between deep learning and mobile networking research is provided in~\cite{zhang2019deep} where the authors discuss how to tailor deep learning to mobile environments. Current challenges and open future research directions are also discussed. 

We stress that that most of the works in the literature, with the exception of~\cite{chen2016automatic,zhang2017zipnet,aceto2018mobile} and~\cite{aceto2019mobile}, classify mobile traffic based on manual feature extraction and all the papers that we surveyed process network or application level data. Our work departs from prior art as we leverage the feature extraction capabilities of deep neural networks and classify mobile data gathered from the physical channel of a mobile operative network, at runtime, and without access to application data and TCP/UDP port numbers.


==> Mobile Data Analysis - Journal/Results.tex <==

\section{Supervised Training and Comparison of Traffic Classification Algorithms}
\label{sec:results}

\input{new_new_table}
\input{new_new_table2}

%In this section we will evaluate the numerical results for both app and service classification problems. First, some metrics to asses our approaches are defined in Section~\ref{sec:metrics}. The performance evaluation over the different metrics is discussed in Section~\ref{sec:perf_ev}. Finally, some details are given about the importance of the session duration in Section~\ref{sec:perf_time}.

The performance tests have been carried out using an Intel core i7 machine, with $32$ GB of RAM and an NVIDIA GTX 980 GPU card. We divided the dataset, featuring $10,000$ labeled DCI sessions, into training and validation sets with a split ratio of \mbox{$70\%$ - $30\%$}. These sets are balanced, as they contain the same percentage of traces for all classes. The classification algorithms have been implemented in Python. We have used \verb|keras| library on top of Tensorflow backend for the implementation of deep NNs. For the benchmark classifiers, we used the popular \verb|sklearn| library.

%\begin{figure*}[ht]
%	\centering
%%	\includegraphics[width=.66\columnwidth]{figures/train_mlp}
%	\includegraphics[width=.8\columnwidth]{figures/train_rnn}
%	\includegraphics[width=.8\columnwidth]{figures/train_cnn}
%	\caption{Accuracy versus number of epochs for training and validation sets in app identification problem.}
%	\label{fig:train_test}
%\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Def. Performance Metrics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Performance Metrics}
\label{sec:metrics}

%The classification performance is assessed through the following metrics: \textit{accuracy} (ratio between the number of correctly classified sessions to the total number of sessions), \textit{precision} (for each class, the ratio between the number of samples belonging to that class that are correctly classified (true positives) and the sum between true positives and false positives), \textit{recall} (for each class, the ratio between the true positives $T_p$ and the sum of true positives and false negatives) and \textit{F-score} the harmonic mean of precision and recall.
The classification performance is assessed through the following metrics:
\begin{enumerate}
\item \textbf{Accuracy}: defined as the ratio between the number of correctly classified sessions to the total number of sessions.
\item \textbf{Precision} $P$: defined, for each class, as the ratio between true positives $T_p$ and the sum between true positives and false positives $F_p$,
\begin{equation}
P = \frac{T_p}{T_p+F_p},
\end{equation}

\item \textbf{Recall} $R$: defined, for each class, as the ratio between the true positives $T_p$ and the sum of true positives and false negatives $F_n$,
\begin{equation}
R = \frac{T_p}{T_p+F_n}.
\end{equation}

\item \textbf{F-Score} $F$ is defined as the harmonic mean of precision $P$ and recall $R$,
\begin{equation}
\displaystyle F = \left(\frac{\frac{1}{P}+\frac{1}{R}}{2}\right)^{-1}=2\frac{RP}{R+P}.
\end{equation}
%F = \left(\frac{P^{-1}+R^{-1}}{2}\right)^{-1}=\frac{2RP}{R+P}
\end{enumerate}
Note that the definition of precision and recall only applies to classification tasks with one class. However, tasks O1 and O2 both have a number of classes $K >2$, namely, $K=\{3,6\}$ for app and service identification, respectively. Thus, precision and recall are separately calculated for all the $K$ classes, and their average is shown in the following numerical results.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Comparison of classification algorithms
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Comparison of Classification Algorithms}
\label{sec:perf_ev}
\subsubsection{Accuracy and Algorithm Training}

Tables~\ref{table_app} and~\ref{table_service} summarize the obtained performance metrics for the deep \acp{NN} and the benchmark classifiers for app and service identification, respectively. First, we focus on synchronous sessions results. In general, better performance is achieved through deep \acp{NN} ($+13.8\%$ on app identification, $+8.7\%$ on service classification). Moreover, we observe a significant performance gap between the service and app classification tasks, due to the higher number of classes of the latter: the performance gap is higher than $8\%$ for the benchmark classifiers and ranges from $2$ to $6\%$ for NNs. Furthermore, \ac{RNN} and \ac{CNN} architectures achieve an accuracy of about $99\%$ for the service identification task (O1) and higher than $95\%$ for the app identification task (O2). The algorithm based on Gaussian Processes performs the best among the benchmark classifiers. In general, the higher the complexity (i.e., the number of parameters, and also hidden layers for NNs), the higher the performance. The only exception to this is provided by \acp{CNN}, which present the highest accuracy but use a small number of parameters. This fact confirms the high efficiency of convolutions in processing high amount of data with complex temporal structure, and the effectiveness of parameter sharing. \acp{CNN} require only $6\%$ of the variables used up by \acp{RNN}, achieving a better accuracy. This also translates into a faster training: in Fig.~\ref{fig:train_test}, we show the accuracy as a function of the number of epochs for training and validation sets for RNNs and CNNs. The number of epochs required by the \acp{CNN} to reach an accuracy higher than $90\%$ is fewer than $20$ (Fig.~\ref{fig:train_test_CNN}), whereas for RNNs convergence is achieved only after $30$ epochs (Fig.~\ref{fig:train_test_RNN}).

\begin{figure*}[t]
	\centering
	\begin{subfigure}[t]{.8\columnwidth}
		\centering
		\includegraphics[width=0.98\columnwidth]{figures/train_rnn_async}
		\caption{RNN.}
		\label{fig:train_test_RNN}	
	\end{subfigure}
	%\quad
	\begin{subfigure}[t]{.8\columnwidth}
		\centering
		\includegraphics[width=0.98\columnwidth]{figures/train_cnn_async}
		\caption{CNN.}
		\label{fig:train_test_CNN}	
	\end{subfigure}
	\centering
	\caption{Accuracy {\it vs} number of epochs for training and validation sets for the app identification task.}
	\label{fig:train_test}
\end{figure*}



%\subsubsection{Training and Convergence of \acp{NN}}

%Regarding the differences between \acp{NN} approaches and the rest of classifiers, the result is as expected: the deeper and more complex architecture, the better the accuracy. However, this entails higher computation times that can be a drawback for certain applications. Moreover, bigger differences can be observed in app classification rather than service identification due to the higher number of possible outputs, and thus higher complexity.

%It should be noted that although the \ac{RNN} and \ac{CNN} approaches perform with similar results, the computation complexity regarding \ac{RNN} is much higher as can be confirmed looking at the number of trainable parameters in Tables~\ref{table_app} and \ref{table_service}. The \ac{CNN} requires just the $6\%$ of variables in comparison with \ac{RNN} to achieve an even better accuracy, which translates into a much faster training phase.

%The accuracy vs the number of epochs is reported in Fig.~\ref{fig:train_test} for both train and validation sets. As can be seen, the number of epochs required to train the \ac{CNN} is relatively low compared to the time needed by the \ac{RNN}: in few epochs (less than $20$), the \ac{CNN} reaches is maximum accuracy (around $97\%$); in contrast, the \ac{RNN} accuracy has more variance and it is unpredictable until $20$ epochs; a relatively stable values are achieved only after $60$ epochs.

%This comes from the \ac{RNN} architecture where more neurons per layer are needed and also the LSTM Memory Cells (\acp{MC}) are more complex than the neurons in \ac{CNN}.

%For these reasons, we propose the \ac{CNN} architecture as the algorithm to classify the user mobile sessions. \trinh{maybe in conclusions}

%\begin{figure}[t]
%	\centering
%	\includegraphics[width=.5\columnwidth]{figures/confusion_service}
%	\caption{Confusion matrix for service identification.}
%	\label{fig:conf_service}
%\end{figure}
%
%\begin{figure}[t]
%	\centering
%	\includegraphics[width=\columnwidth]{figures/confusion_app}
%	\caption{Confusion matrix for app identification.}
%	\label{fig:conf_app}
%\end{figure}

%\bigskip
\subsubsection{Confusion Matrix}

A deeper look at the performance of CNNs is provided by the confusion matrices of Fig.~\ref{fig:conf_matrices}, whose rows and columns respectively represent true and predicted labels, and all values are normalized between $0$ and $1$. For the service classification task (Fig.~\ref{fig:conf_service}), CNNs only misclassify the video streaming sessions: $2\%$ of those are labeled as video calls. For the app identification task (Fig.~\ref{fig:conf_app}), errors ($4\%$) mainly occur for Skype and WhatsApp videocalls. These errors are understandable, as these are both interactive real-time video applications and, as such, their traffic patterns bear similarities. The lowest performance is found for Vimeo traces, for which $88\%$ of the sessions are correctly classified. Here our CNN-based classifier confuses them with the other video applications for both streaming service (Youtube - $3\%$) and real-time calling (WhatsApp and Skype - $6\%$ and $3\%$, repectively).
\begin{figure*}[h]
	\centering
	\begin{subfigure}[t]{.8\columnwidth}
		\centering
		\includegraphics[width=0.98\columnwidth]{figures/confusion_service}
		\caption{Confusion matrix for service identification.}
		\label{fig:conf_service}	
	\end{subfigure}
	%\quad
	\begin{subfigure}[t]{.8\columnwidth}
		\centering
		\includegraphics[width=0.98\columnwidth]{figures/confusion_app}
		\caption{Confusion matrix for app identification.}
		\label{fig:conf_app}	
	\end{subfigure}
	\centering
	\caption{Confusion matrices for the \ac{CNN} algorithm.}
	\label{fig:conf_matrices}
\end{figure*}
%The confusion matrix of the \ac{CNN} classifier is shown in Fig.~\ref{fig:conf_matrices}. A confusion matrix is a table that describes the performance of a classification model over a labeled dataset, where each row of the matrix represents the instances in a predicted class, while each column represents the instances in an actual class (or viceversa). In this case, each row represents the true labels while each column shows the sessions classified as a certain class type (app or service), i.e., the predicted labels. All values shown in Fig.~\ref{fig:conf_matrices} are normalized between $0$ and $1$. Regarding Fig.~\ref{fig:conf_service}, it can be seen that there are no errors in the prediction except for just a $2\%$ of the video streaming sessions which are classified as video calls. As for Fig.~\ref{fig:conf_app}, some errors (just the $4\%$) in the prediction can be found in the pair of classes Skype and Whatsapp video, in which sessions belonging to Skype are classified as Whatsapp videos and vice versa. These are comprehensible errors, since the sessions' classes are both video applications. The lowest performance is found in the Vimeo traces, where the $88\%$ of the sessions are correctly classified. The evaluation of the rest of metrics, i.e., precision, recall and $F$-Score is included in Tables~\ref{table_app} and \ref{table_service}. %A comparison of these metrics for all classifiers in the app identification is presented in Fig.~\ref{fig:precision_recall}.
%Similarly to the accuracy, the best \mbox{$F$-Score} is obtained by the \ac{CNN}.

%\begin{figure}[t]
%\centering
%\includegraphics[width=\columnwidth]{figures/precision_recall}
%\caption{Precision and recall comparison for app classification. $F$-Score is shown on top of the bars.}
%\label{fig:precision_recall}
%\end{figure}

\subsubsection{Asynchronous Sessions Results}


As shown in the last two columns of Tables~\ref{table_app} and~\ref{table_service}, the algorithms' accuracy is affected by asynchronous sessions. As expected, we observe a general decrease in the accuracy for all the algorithms ($-6.0\%$ for service identification, $-7.7\%$ for app identification, on average). However, for both classification problems, neural network-based approaches are more robust to the asynchronous case, showing a performance degradation of $-4.3$\%, while the degradation of standard algorithms is $-8.4$\%.

\subsubsection{Impact of Different Window Sizes}
Fig.~\ref{fig:accuracy_vs_W} shows the classification accuracy as a function of the window size, $W$. For the app identification task, $40$~seconds suffice for \acp{CNN} and \acp{RNN} to reach accuracies higher than $90\%$, with negligible additional improvements for longer observation periods. Periods shorter than $40$ seconds provide less accurate results. Similar trends are observed for the service classification task. However, in this case after $20$ seconds the accuracy of \acp{CNN} and \acp{RNN} is already higher than $90\%$, due to the smaller number of classes. In summary, the ability of \acp{CNN} and \acp{RNN} to extract representative statistical features from a session grows with the input data length. In our tasks, deep NN algorithms become very effective as monitoring intervals get longer than $20$ seconds. 

%\subsection{Performance vs Session Length}
%\label{sec:perf_time}

%With Fig.~\ref{fig:accuracy_vs_time}, we gauge the relationship between session monitoring time and accuracy. For the app identification task, $80$ seconds suffice for \acp{CNN} to achieve their highest accuracy, while longer observation periods lead to negligible performance improvements. Observation periods shorter than $20$ seconds give less accurate results, and low complexity algorithms (e.g., MLP) perform the best in this case. Similar trends are observed for the service classification task. However, in this case after $50$ seconds the accuracy of \acp{CNN} and \acp{RNN} is already close to $99\%$, due to the smaller number of classes. In summary, the ability of \acp{CNN} and \acp{RNN} to extract representative statistical features from a session grows with the input data length. In our tasks, deep NN algorithms become very effective as monitoring intervals get longer than $20$ seconds.
\begin{figure*}[t]
	\centering
	\begin{subfigure}[t]{.8\columnwidth}
		\centering
		\includegraphics[width=0.98\columnwidth]{figures/sync_async_app}
		\caption{App identification.}
		\label{fig:sync_async_app}	
	\end{subfigure}
	%\quad
	\begin{subfigure}[t]{.8\columnwidth}
		\centering
		\includegraphics[width=0.98\columnwidth]{figures/sync_async_service}
		\caption{Service identification.}
		\label{fig:sync_async_app_service}	
	\end{subfigure}
	\centering
	\caption{
		Effect of Synchronization vs Asynchronization procedures}
	\label{fig:sync_async_app}
\end{figure*} 

\begin{figure*}[t]
	\centering
	\begin{subfigure}[t]{.8\columnwidth}
		\centering
		\includegraphics[width=0.98\columnwidth]{figures/bench_vs_W_app}
		\caption{Accuracy for app identification.}
		\label{fig:bench_vs_W_app}	
	\end{subfigure}
	%\quad
	\begin{subfigure}[t]{.8\columnwidth}
		\centering
		\includegraphics[width=0.98\columnwidth]{figures/bench_vs_W_service}
		\caption{Accuracy vs Window Size $W$ for service identification.}
		\label{fig:bench_vs_W_service}	
	\end{subfigure}
	\centering
	\caption{
	Accuracy {\it vs} window lengths for app and service classification tasks.}
	\label{fig:accuracy_vs_W}
\end{figure*} 

%The assessment of the accuracy performance with respect to the session duration is shown in Fig.~\ref{fig:accuracy_vs_time} for both problems. This evaluation allows us to know after how much time a classifier can perform the service/app classification reaching a certain accuracy. Accordingly, this analysis indicates for how much time we need to sniff the LTE control channel before being able to classify a certain session pattern.

%The session duration corresponds to the number of samples $N$ per session that composes the dataset matrix $\bm{X}$ (see Section~\ref{sec:problem}). It can be observed that to achieve an accuracy of $90\%$ in the app identification, at least $60$ seconds are needed using the proposed \ac{CNN} architecture. Below this session interval, the MLP and even the linear SVM perform better than \ac{CNN} and \ac{RNN}, but the obtained accuracies are far inferior than the top performance.

%The same trend is observable also in the service identification problem: also in this case the MLP perform better at the beginning, but to achieve an accuracy of $90\%$, we require only $20$ seconds, since the service can be identified more easily with respect to the app. In this case, after $30$ seconds, the \ac{CNN} and \ac{RNN} performance are close to $100\%$.

%The motivation for these results are intrinsically due to the \mbox{NN-structures}: the ability of \ac{CNN} and \ac{RNN} to extract the time correlations between samples within a trace, generally, grows with the input data size. As can be seen in Fig.~\ref{fig:accuracy_vs_time}, implying NN algorithms for high accuracy classification becomes advantageous only when considering more than $20$ seconds.

%\begin{figure}[t]
%\centering
%\includegraphics[width=\columnwidth]{figures/accuracy_vs_time}
%\caption{Accuracy for app identification.}
%\label{fig:accuracy_vs_time}
%\end{figure}


==> Mobile Data Analysis - Journal/Supervised_Learning_Approach.tex <==
%!TEX root = main.tex

\section{Supervised Learning}
\label{sec:sl}

In this section, we present several supervised \ac{ML} algorithms that are used as benchmarks for the two classification problems: for the sake of clarity, we distinguish two classes of classification algorithms, whether they include a \mbox{\ac{NN}-based} structure or not. Details about the \mbox{\ac{NN}-based ones} are given in Section~\ref{sec:nn}. The other group of classifiers are presented as follows. 

\subsection{Linear Classifiers}
For this type of algorithms, we choose a linear \ac{SVM} and logistic regression. Both are discriminative models, which means that they try to model by just depending on the observed data while learning how to do the classification. Unlike generative models, a discriminative model makes fewer assumptions on the distributions but depends heavily on the quality of the data. 

Generally, given a linear classifier, if the input feature vector is ${\bm{x}}$, then the output score  is: 
\begin{equation}
\bm{y}=f({\bm{w}}\cdot {\bm {x}})=f\left(\sum _{j}w_{j}x_{j}\right)
\end{equation}	

\subsubsection{Linear Logistic Regression} Although this algorithm derives from linear regression, it can be used to perform classification. In linear regression, the output  is modeled as a linear combination of features: $\bm{y} = \sum _{j}w_{j}x_{j} + b$. Differently, in logistic regression, in a binary case, is the probability of the output that is modeled as a linear combination of the features. The following is also called Logit function: 
\begin{equation}
log\left(\frac{\pi}{1-\pi}\right) = \sum _{j}w_{j}x_{j}+b
\end{equation}

where $\pi$, in a binary case, is the probability of $\bm{x}$ to belong to one of the two class. It follows that $\pi$ is given by:
\begin{equation}
\pi = \frac{e^{\sum _{j}w_{j}x_{j} + b}}{1+e^{\sum _{j}w_{j}x_{j} + b}}=
\frac{1}{1+e^{-{\sum _{j}w_{j}x_{j} + b}}},
\end{equation}
which is the Logistic function. For this reason, this classifier represents a particular case of a linear model, since it is the probability of belonging to a class that is modeled as a linear combination and not the actual output. In our problem, we adopt the implementation from the library presented in~\cite{fan2008liblinear}.

\subsubsection{Linear SVM} Support vector machines defines hyperplanes to separate the input data in the features vector space, maximizing the margin around the separating hyperplane. The decision function is fully specified by a small subset of training samples, the support vectors. 

In our problem, we use a linear SVM classifier to identify the different mobile apps. In our implementation, we use the Hinge loss function~\cite{wu2007robust} to compute the \mbox{maximum-margin} classification. We use a standard L2-norm for regularization with the penalty parameter $C=0.025$. The library implementation details can be found here\cite{chang2011libsvm}.
% For the loss, we use the Hinge loss function \angel{(Add ref here)} to compute the \mbox{maximum-margin} classification.
%\begin{equation}
%L(y)=\max(0,1-t\cdot y)
%\end{equation}
%where $y$ is the classifier score and $t\in \left(0,1\right)$ is the intended output. 
\mbox{Non-linear} SVM can be implemented by applying a kernel function instead of the matrix multiplication, but the kernel selection and the analysis to obtain non linearities deserves a separate study. \\


Both linear methods are originally intended for binary classification, but the extension from the binary case to a \mbox{multi-class} classification can be done using the \mbox{one-vs-all} scheme~\cite{fan2008liblinear}.

\subsection{Random Forest} Random forest is an ensemble learning method, which operates by constructing a multitude of decision trees at training time, and outputting the predicted class, i.e., service or app type, of the input user session. With respect to larger decision trees, random forests are less prone to overfitting over the training dataset. Thus, random forests are used to average multiple deep decision trees, with the goal of reducing the variance, generally boosting the accuracy in the final model.

Formally, the random forest consists of a collection of tree-structured classifiers $h(\bm{X},\theta_{n_t})$ with $n_t=1, ..., N_T$, $N_T$ number of trees, and $\theta_{n_t}$ are independent identically distributed random vectors, which account for the random choices we make when fitting the $n_t$-th tree~\cite{breiman2001random}. In our work, we choose $N_T=10$ and we use the bootstrap technique (also known as \textit{bagging}) for the random choices. Given $M$ the total number of sessions, $\bm{y}$ the output class vector and $N_T$ the total number of trees, the bagging technique for random sampling applies as follows:
\begin{algorithm}[h]
\SetAlCapSkip{2em}
 \For{$n_t = 1 \dots N_T$}{
 {
 \begin{itemize}[leftmargin=*]{
 \itemsep0.5em 
  \item sample, with replacement, $M$ training examples from $\bm{X}, \bm{y}$; these are $X_{n_t}, \bm{y}_{n_t}$\;
  \item train the classification tree $h(\bm{X},\theta_{n_t})$ on  $X_{n_t}, \bm{y}_{n_t}$\; 
 }
 \end{itemize}
  }
 }
 \caption{Bootstrap procedure for random forests.}
\end{algorithm}

\subsection{Gaussian Processes} 
%Bayesian \mbox{non-parametric} models, such as Gaussian Processes (GPs), can represent beliefs about the model parameters via a probability distribution (called the {\it prior} distribution). Then, Bayesian inference can reshape the prior distribution, transforming it into a {\it posterior} one. GPs have become popular for regression and classification, often showing impressive empirical performance.

%A GP is a generalization of the Gaussian probability distribution and can be used for probabilistic classification. Formally, a GP is a collection of random variables, any finite number of which have a joint Gaussian distribution and it is completely specified by the mean function $m(x)$ and the covariance function $k(x, \hat x)$ .
%\begin{equation}f(\cdot) \sim GP(m(x), k(x, \hat x))\end{equation} 


%For a binary classification task, we need to predict the probability $\pi(x)$, which lies in $[0,1]$:  the basic idea behind the Gaussian process prediction is to place a GP prior over the latent function $f(x)$ and then squash $f(x)$ through any sigmoid function to obtain a prior on $\pi(x) = \sigma(f(x))$. The latent function is a so-called nuisance function, whose values are not observed and are not relevant by themselves. Its purpose is to allow a convenient formulation of the model, and  is removed during prediction. Generally, the Logistic function is used to squash $f(x)$.

%In contrast to a regression task, the posterior of the latent function $\pi(x)$ is not Gaussian even for a GP prior because of discrete class labels. Rather, a non-Gaussian likelihood corresponding to the logistic function is used. The approximation of the non-Gaussian posterior with a Gaussian likelihood is done by using the Laplace approximation. The details of the GP implementation can be found in~\cite{rasmussen2004gaussian}.

Gaussian Processes (GPs) are a \mbox{non-parametric} approach that aims to find a distribution over all the possible functions $f(x)$ that are consistent with the observed data. As with all Bayesian methods, it begins with a prior distribution which is updated as data points are observed, producing the posterior distribution over functions.

Although to represent a distribution over a set of possible functions can be difficult, it turns out that only a distribution over the function's values at a finite, but arbitrary, set of points is needed. Formally, a GP is a collection of random variables, any finite number of which have a joint Gaussian distribution and it is completely specified by the mean $\mu(x)$ and covariance function $\Sigma(x)$:

\begin{equation}
f(\cdot) \sim GP(\mu(x), \Sigma(x)).
\end{equation} 

As described in~\cite{rasmussen2004gaussian}, GPs can be used for classification tasks, finding a probability $\pi(x)$ that lies in $[0,1]$: the basic idea behind is to place a prior Gaussian distribution over the latent function $f(x)$ and then squash $f(x)$ through any sigmoid function to obtain a prior on $\pi(x) = \sigma(f(x))$. The latent function is a \mbox{so-called} nuisance function, whose values are not observed and are not relevant by themselves. Its purpose is to allow a convenient formulation of the model, and is removed during prediction. In our work, the Logistic function is used to squash $f(x)$. The details of the GP implementation can be found in~\cite{rasmussen2004gaussian}.


==> Mobile Data Analysis - Journal/new_new_table.tex <==
%%!TEX root = main.tex
\begin{table*}[t]
\centering
\ra{0.5}
\footnotesize
\begin{tabular}{*{8}{c}}
\textbf{Algorithm}&\multicolumn{1}{c}{\textbf{Accuracy $\%$}} & \multicolumn{1}{r}{\textbf{Precision}} & \textbf{Recall} & \textbf{F-Score} & \textbf{\# Parameters}  & \textbf{Acc Async $\%$} & \textbf{Diff $\%$} \\
\midrule
\rowcolor{black!5} Linear SVM & 81.23 & 0.811 & 0.812 & 0.805  & 36726 & 68.41 & -12.8\\
\rowcolor{black!0}Logistic Regressor & 81.61 & 0.806 &0.816& 0.809   &  486 & 65.72 & -15.9 \\
\rowcolor{black!5}Nearest Neighbours   & 84.51 & 0.843 &0.845& 0.841   &   36720 & 79.65 & -4.9\\
\rowcolor{black!0}Random Forest  & 83.52 & 0.821& 0.835& 0.827  &   41310 & 70.21 & -13.3\\
\rowcolor{black!5}Gaussian Processes  & 87.43 & 0.874 & 0.871  & 0.871   &   146720 & 81.21 & -6.2\\
\midrule
\textbf{Neural Networks} &  &   &    &    &  \\
\midrule
\rowcolor{black!5}MLP & 90.04 & 0.900 & 0.900 & 0.900  &  19014 & 84.61 & -5.4 \\
\rowcolor{black!0} RNN  &  96.57 & 0.967  & 0.968   & 0.968  & 392046  & 92.93 & -3.6\\
\rowcolor{black!5}CNN & 97.77 & 0.978 & 0.976  & 0.977   & 25062 & 93.20 & -4.5\\
\bottomrule

\end{tabular}

\caption{Classifiers comparison for the app identification task.}
\label{table_app}
\end{table*}


==> Mobile Data Analysis - Journal/new_new_table2.tex <==
%!TEX root = main2.tex
\begin{table*}[t]
\centering
\ra{0.5}
\footnotesize
\begin{tabular}{*{8}{c}}
\textbf{Algorithm}&\multicolumn{1}{c}{\textbf{Accuracy $\%$}} & \multicolumn{1}{r}{\textbf{Precision}} & \textbf{Recall} & \textbf{F-Score} & \textbf{\# Parameters} & \textbf{Acc Async $\%$} & \textbf{Diff $\%$} \\
\midrule
\rowcolor{black!5} Linear SVM & 90.80 & 0.908& 0.908& 0.907  &  19843 & 79.61  & -11.2\\
\rowcolor{black!0}Logistic Regressor & 90.42 & 0.904& 0.904& 0.904   & 243 & 81.11 & -9.3\\
\rowcolor{black!5}Nearest Neighbours   & 92.76 & 0.925& 0.925& 0.925 &  19840 & 83.45 & -9.3\\
\rowcolor{black!0}Random Forest  & 91.57 & 0.915& 0.915& 0.915 &  22320 & 84.25 & -7.3\\
\rowcolor{black!5}Gaussian Processes  &  93.21 & 0.932 & 0.928 & 0.929 &  73360 & 82.51 & -10.7\\
\midrule
\textbf{Neural Networks} &  &   &    &    & \\
\midrule
\rowcolor{black!5}MLP &  94.31 & 0.943 & 0.939 & 0.942  & 18819 & 93.38 & -0.9 \\
\rowcolor{black!0} RNN  &  98.21 & 0.981 & 0.982 & 0.981 & 391503 & 95.38 & -2.8\\
\rowcolor{black!5}CNN & 98.87 & 0.986 & 0.988 & 0.988  & 24963 & 95.40 & -3.5\\
\bottomrule
\end{tabular}
\caption{Classifiers comparison for the service identification task.}
\label{table_service}

\end{table*}

==> Mobile Data Analysis - Journal/new_table.tex <==
%%!TEX root = main.tex
\begin{table*}[t]
\centering
\ra{0.7}
\trinh{

\begin{tabular}{*{8}{c}}\toprule

\textbf{Algorithm}&\multicolumn{1}{c}{\textbf{Accuracy $\%$}} & \multicolumn{1}{r}{\textbf{Precision}} & \textbf{Recall} & \textbf{F-Score} & \textbf{\# Parameters}  & \textbf{Acc Async $\%$} & \textbf{Diff $\%$} \\
\midrule
\rowcolor{black!5} Linear SVM & 80.07 & 0.815 & 0.801 & 0.801   & 36726 & 64.34 & -15.8\\
\rowcolor{black!0}Logistic Regressor & 74.84 & 0.741 & 0.748  & 0.748   &  486 & 63.23 & -11.6 \\
\rowcolor{black!5}Nearest Neighbours   & 77.78 & 0.797 & 0.778  & 0.778   &   36720 & 76.56 & -1.2 \\
\rowcolor{black!0}Random Forest  & 77.12 & 0.813 & 0.771  & 0.760   &   41310 & 68.41 & -8.7\\
\rowcolor{black!5}Gaussian Processes  & 86.93 & 0.873 & 0.869  & 0.869   &   146720 & 79.08 & -7.8\\
\midrule
\textbf{Neural Networks} &  &   &    &    &  \\
\midrule
\rowcolor{black!5}MLP & 86.27 & 0.866  &  0.863  & 0.860  &  19014 & 81.16 & -5.1 \\
\rowcolor{black!0} RNN  &  95.37 & 0.956  & 0.954   & 0.954  & 392046  & 90.05 & -5.3\\
\rowcolor{black!5}CNN & 97.83 & 0.978 & 0.978  & 0.978   & 25062 & 91.48 & -6.4\\
\bottomrule

\end{tabular}
}
\caption{Classifiers comparison for the app identification task.}
\label{table_app}
\end{table*}




==> Mobile Data Analysis - Journal/new_table2.tex <==
%!TEX root = main.tex
\begin{table*}[t]
\centering
\ra{0.7}
\trinh{

\begin{tabular}{*{8}{c}}\toprule

\textbf{Algorithm}&\multicolumn{1}{c}{\textbf{Accuracy $\%$}} & \multicolumn{1}{r}{\textbf{Precision}} & \textbf{Recall} & \textbf{F-Score} & \textbf{\# Parameters} & \textbf{Acc Async $\%$} & \textbf{Diff $\%$} \\
\midrule
\rowcolor{black!5} Linear SVM & 87.58 & 0.877 &  0.875 & 0.871  &  19843 & 78.51  & -9.0\\
\rowcolor{black!0}Logistic Regressor & 87.58 & 0.883 & 0.875 & 0.877   & 243 & 79.28 & -8.3\\
\rowcolor{black!5}Nearest Neighbours   & 82.67 & 0.850 & 0.826 & 0.833 &  19840 & 81.56 & -1.1\\
\rowcolor{black!0}Random Forest  & 89.54 & 0.915 & 0.895 & 0.901 &  22320 & 81.27 & -8.3\\
\rowcolor{black!5}Gaussian Processes  &  92.81 & 0.932 & 0.928 & 0.928 &  73360 & 80.78 & -12.0\\
\midrule
\textbf{Neural Networks} &  &   &    &    & \\
\midrule
\rowcolor{black!5}MLP &  92.81 & 0.930 & 0.928 & 0.929  & 18819 & 91.31 & -1.5 \\
\rowcolor{black!0} RNN  &  98.14 & 0.981 & 0.982 & 0.981 & 391503 & 94.46 & -3.7\\
\rowcolor{black!5}CNN & 99.07 & 0.986 & 0.994 & 0.989  & 24963 & 95.39 & -3.7\\
\bottomrule
\end{tabular}
}
\caption{Classifiers comparison for the service identification task.}
\label{table_service}

\end{table*}

==> Mobile Data Analysis - Journal/table.tex <==
%%!TEX root = main.tex
\begin{table*}[t]
\centering
\ra{0.7}

\begin{tabular}{*{6}{c}}\toprule
\textbf{Algorithm}&\multicolumn{1}{c}{\textbf{Accuracy $\%$}} & \multicolumn{1}{r}{\textbf{Precision}} & \textbf{Recall} & \textbf{F-Score} & \textbf{\# Parameters}  \\
\midrule
\rowcolor{black!5} Linear SVM & 80.07 & 0.815 & 0.801 & 0.801   & 36726 \\
\rowcolor{black!0}Logistic Regressor & 74.84 & 0.741 & 0.748  & 0.748   &  486 \\
\rowcolor{black!5}Nearest Neighbours   & 77.78 & 0.797 & 0.778  & 0.778   &   36720\\
\rowcolor{black!0}Random Forest  & 77.12 & 0.813 & 0.771  & 0.760   &   41310\\
\rowcolor{black!5}Gaussian Processes  & 86.93 & 0.873 & 0.869  & 0.869   &   146720\\
\midrule
\textbf{Neural Networks} &  &   &    &    &  \\
\midrule
\rowcolor{black!5}MLP & 86.27 & 0.866  &  0.863  & 0.860  &  19014  \\
\rowcolor{black!0} RNN  &  95.37 & 0.956  & 0.954   & 0.954  & 392046  \\
\rowcolor{black!5}CNN & 97.83 & 0.978 & 0.978  & 0.978   & 25062 \\
\bottomrule
\end{tabular}
\caption{Classifiers comparison for the app identification task.}
\label{table_app}
\end{table*}




==> Mobile Data Analysis - Journal/table2.tex <==
%!TEX root = main.tex
\begin{table*}[t]
\centering
\ra{0.7}

\begin{tabular}{*{6}{c}}\toprule
\textbf{Algorithm}&\multicolumn{1}{c}{\textbf{Accuracy $\%$}} & \multicolumn{1}{r}{\textbf{Precision}} & \textbf{Recall} & \textbf{F-Score} & \textbf{\# Parameters} \\
\midrule
\rowcolor{black!5} Linear SVM & 87.58 & 0.877 &  0.875 & 0.871  &  19843\\
\rowcolor{black!0}Logistic Regressor & 87.58 & 0.883 & 0.875 & 0.877   & 243\\
\rowcolor{black!5}Nearest Neighbours   & 82.67 & 0.850 & 0.826 & 0.833 &  19840\\
\rowcolor{black!0}Random Forest  & 89.54 & 0.915 & 0.895 & 0.901 &  22320\\
\rowcolor{black!5}Gaussian Processes  &  92.81 & 0.932 & 0.928 & 0.928 &  73360\\
\midrule
\textbf{Neural Networks} &  &   &    &    & \\
\midrule
\rowcolor{black!5}MLP &  92.81 & 0.930 & 0.928 & 0.929  & 18819  \\
\rowcolor{black!0} RNN  &  98.14 & 0.981 & 0.982 & 0.981 & 391503 \\
\rowcolor{black!5}CNN & 99.07 & 0.986 & 0.994 & 0.989  & 24963\\
\bottomrule
\end{tabular}
\caption{Classifiers comparison for the service identification task.}
\label{table_service}
\end{table*}

==> Mobile Data Analysis - Journal/table_params.tex <==
\begin{table}[t]
\centering
\caption{Configuration parameters for the benchmark classifiers.}
\ra{0.5}
\scriptsize
\begin{tabular}{p{1.2cm}p{2.4cm}p{3.1cm}}\toprule
\textbf{Algorithm}&\hspace{0.2cm}\textbf{Parameters}& \hspace{0.2cm}\textbf{Note - Reference} \\
\midrule
\rowcolor{black!5} Linear SVM & \begin{tabular}{p{2.4cm}}
\tabitem \textit{penalty} = L2 \\
\tabitem \textit{loss} = Hinge Loss \\
\tabitem $c = 0.025$
\end{tabular} & \begin{tabular}{p{3.1cm}}
\tabitem $c$: penalty parameter for the error term\\
\tabitem extended to multi-class with one-vs-rest~\cite{fan2008liblinear}
\end{tabular}\\
\midrule
\rowcolor{black!0} Logistic Regressor& \begin{tabular}{p{2.4cm}}
\tabitem \textit{penalty} = L2 \\
\tabitem $c = 1$
\end{tabular} & \begin{tabular}{p{3.1cm}}
\noindent \tabitem $c$: inverse of the regularization strength\\
\tabitem extended to multi-class with one-vs-rest~\cite{fan2008liblinear}
\end{tabular}\\
\midrule
\rowcolor{black!5} Nearest Neighbours & \begin{tabular}{p{2.4cm}}
\tabitem $K = 3$\\
\tabitem $p = 2$\\
\tabitem \textit{metric} = Minkowski   
\end{tabular} & \begin{tabular}{p{3.1cm}}
\tabitem $K$: number of neighbors for queries\\ 
\tabitem $p$: distance metric parameter\\
\tabitem $p = 2$ amounts to using the Euclidean distance~\cite{altman1992introduction}
\end{tabular}\\
\midrule
\rowcolor{black!0 } Random Forest & \begin{tabular}{p{2.4cm}}
\tabitem \textit{n. estimators} $= 10$\\
\tabitem \textit{max depth} $= 5$\\
\tabitem \textit{criterion} $=$ entropy\\
\end{tabular} & \begin{tabular}{p{3.1cm}}
\tabitem \textit{n. estimators}: number of trees in the forest\\ 
\tabitem  \textit{max depth}: maximum depth of a tree\\
\tabitem  \textit{criterion}: function to measure the quality of a split of subsets~\cite{breiman2001random}\\
\end{tabular}\\
\midrule	
\rowcolor{black!5} Gaussian Processes & \begin{tabular}{p{2.4cm}}
\tabitem \textit{kernel} $=$ RBF\\
\tabitem $\sigma =$ Logistic func.\\
\tabitem \textit{approx.} $=$ Laplacian
\end{tabular} & \begin{tabular}{p{3.1cm}}
\tabitem Radial Basis Function (RBF) used as kernel\\ 
\tabitem $\sigma$ is the sigmoid function used to ``squash'' the nuisance function\\ 							
\tabitem Laplacian method used to approximate the non Gaussian Posterior~\cite{rasmussen2004gaussian}	
\end{tabular}\\
\bottomrule
\end{tabular}
\label{table_params}
\end{table}


==> Mobile Data Analysis - Journal/use_case.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Traffic Profiling
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Unsupervised Traffic Profiling}
\label{sec:traffic_profilig}

Next, we analyze the mobile traffic exchanged within the four selected cell sites (see Section~\ref{sec:unlabeled_dataset}). The traffic load is modeled in terms of aggregated traffic dynamics and type of service requests over the $24$ hours of a day. The identification of mobile traffic, for each of the considered services, is performed using the trained classifiers from Section~\ref{sec:sl} with the {\it unlabeled} dataset. Formally, for each \ac{eNodeB}, the corresponding unlabeled dataset is stored into the tensor $\bm{X}^\prime$, with size $M^\prime \times N \times D$, where $M^\prime$ corresponds to the number of monitored \acp{RNTI} (sessions,  $N$ to the number of collected samples per session and $D=2$ is the number of communications directions (downlink and uplink). Given $\bm{X}^\prime$, as input, the classifier $c$ computes the output $\bm{Y}^\prime$, whose analysis provides a detailed characterization of the mobile user requests for the \ac{eNodeB} within the monitored time span. Vectors $\bm{x}^\prime_m$ and $\bm{y}^\prime_m = c(\bm{x}^\prime_m)$ respectively indicate the \mbox{$m$-th} sample of $\bm{X}^\prime$ and $\bm{Y}^\prime$. In this paper, we restrict our attention to the unsupervised classification of services, and use the \ac{CNN} classifier, as it yields the highest accuracy.

\subsection{Aggregated Traffic Analysis}



Fig.~\ref{fig:aggregate_traffic} shows the {\it aggregated} traffic demand for the four selected \acp{eNodeB} over the $24$ hours of a typical day, where each curve has been normalized with respect to the maximum traffic peak occurred during the day for the corresponding \ac{eNodeB}.
\begin{figure}[h]
	\centering
	\includegraphics[width=.8\columnwidth]{figures/aggregate_traffic_4eNB}
	\caption{Daily Aggregated Traffic for the four eNodeBs.}
	\label{fig:aggregate_traffic}
\end{figure}
The four traffic profiles have a different trend, which depends on the characteristics of the served area (demographics, predominant land use, etc.), as confirmed by~\cite{furno2017tale}. \textbf{PobleSec} is a residential neighborhood and, as such, presents traffic peaks during the evening, at 5 and 11~pm. \textbf{Born} is instead a downtown district with a mixed residential, transport and leisure land use. Two peaks are detected: the highest is at lunchtime around 2~pm, whereas the second one is at dinner time, from 9~pm. This traffic behavior is likely due to the many restaurants and bars in the area. \textbf{CampNou} is mainly residential and presents a similar profile to PobleSec. However, Barcelona FC stadium is located in this area, and three football matches took place during the monitored period (events started at 8:45~pm and ended at 10:45~pm). As expected, a higher traffic intensity is observed during the football match hours. In particular, we registered a high amount of traffic exchanged between $7$~pm to $1$~am, i.e., before, during and after the events. This behavior is probably due to the movement of people attending the matches. \textbf{Castelldefels} is a suburban and low populated area with a university campus. The traffic variation suggests a typical office profile with traffic peaks at 10~am and 5~pm. However, in this radio cell the amount of traffic exchanged is the lowest observed across all \ac{eNodeB} sites, i.e., $6.8$~Gb/hour in the peak hours. The highest traffic intensity was measured in Camp Nou, reaching a peak of $106.1$~Gb/hour ($29.5$~Mb/s on average). Intermediate peak values are detected in Poble Sec and Born, amounting to $49.7$~Mb/s and $46.1$~Mb/s, respectively. The only common pattern among the four areas is the low traffic intensity at night, between $2$~am and $7$~am.


\subsection{Traffic Decomposition at Service Level}

The set of applications that we have labeled is restricted to those apps and services that dominate the radio resource usage. However, additional apps may also be present in the monitored traffic, such as Facebook, Instagram, Snapchat, etc. These apps generate mixed content, including \mbox{audio-streaming}, \mbox{video-streaming} and \mbox{video-calling}. Additional service types may also be generated by, e.g., \mbox{web-browsing} and file downloading. While in the present work the classifiers were not trained to specifically track these apps, for a robust classification outcome, it is desirable that the audio and video streams that they generate will either be captured and classified into the correct service class, or at least flagged as unknown. To locate those traffic patterns for which our classifier may produce inaccurate results, in our analysis we additionally account for the detection of \mbox{out-of-distribution (OOD)} sessions, i.e., of DCI traces that show different traffic dynamics from those learned at training time. To identify these ``statistical outliers'', the DCI data from each new session, $\bm{x}^\prime_m$, is fed to the \ac{CNN} and the corresponding softmax output vector \mbox{$\bm{y}^\prime_m = [y^\prime_{m1}, \dots, y^\prime_{mK}]^T$} is used to discriminate whether $\bm{x}^\prime_m$ is OOD or not, following the rationale in~\cite{hendrycks2018deep}\cite{sigurdsson2002outlier}. In detail, the \mbox{$k$-th} softmax output corresponds to the probability estimate that a given input session $\bm{x}^\prime_m$ belongs to class $k$, i.e., \mbox{$y^\prime_{mk} =\textrm{Prob}(\bm{x}^{\prime}_m \in \text{class \textit{k}})$}, with $k=1,\dots,K$. The classifier chooses the class $k^\star$ that maximizes this probability, i.e., 
\begin{equation}
\label{eq:kstar}
k^\star = \arg\!\max_k y^\prime_{mk}.
\end{equation} 
If a new app, not considered in the training phase, generates sessions having similar characteristics to those in the training set, namely, \mbox{audio-streaming}, \mbox{video-streaming} or real time \mbox{video-calls}, we expect the \ac{CNN} to generalize well and return similar vectors at the output of the softmax layer. That is, the softmax vector that is outputted at runtime for the new app should be sufficiently ``close'' to the output learned by the classifier from the labeled dataset, as the new signal bears statistical similarities with those learned in the training phase. In this case, it makes sense to accept the session and classify it as belonging to class $k^\star$. Otherwise, the session would be classified as OOD.

The problem at hand, boils down to assessing whether the softmax output $\bm{y}^\prime_m$ belongs to the statistical distribution learned by the \ac{CNN} or it is an outlier. This amounts to performing outlier detection in a multivariate setting, with $\bm{y}^\prime_m \in [0,1]^K$, $\sum_k y^\prime_{mk} = 1$. Among the many algorithms that can be used to this purpose, we adopt the method based on Kernelized Spatial Depth (KSD) functions of~\cite{Chen-2009} as it is lightweight and does not require the direct estimation of the probability density function (pdf) of the softmax output layer, which is a critical point, as good estimates require training over many points. Briefly, for a vector $\bm{y} \in \mathbb{R}^K$, we define the spatial sign function as $S(\bm{y}) = \bm{y}/\|\bm{y}\|$ if $\bm{y} \neq \bm{0}$ and $S(\bm{y}) = \bm{0}$ if $\bm{y}=\bm{0}$, where $\| \bm{y} \| = (\bm{y}^T \bm{y})^{1/2}$ is the \mbox{norm-2}. If $\mathcal{Y}_k$ is a training set containing $\ell$ softmax output vectors for a certain class $k$, $\mathcal{Y}_k = \{\bm{y}^{(k)}_1, \bm{y}^{(k)}_2, \dots, \bm{y}^{(k)}_\ell \}$, the {\it sample spatial depth} associated with a new softmax output vector $\bm{y}^\prime_m$ is:
\begin{equation}
\label{eq:spatial_depth}
D(\bm{y}^\prime_m,\mathcal{Y}_k) = 1 - \frac{1}{|\mathcal{Y}_k \cup \bm{y}^\prime_m|-1} \left \|\sum_{\bm{y} \in \mathcal{Y}_k} S(\bm{y}-\bm{y}^\prime_m) \right \| .
\end{equation}
Note that $D(\bm{y}^\prime_m,\mathcal{Y}_k) \in [0,1]$ provides a {\it measure of centrality} of the new point $\bm{y}^\prime_m$ with respect to the points in the training set $\mathcal{Y}_k$. In particular, if $D(\bm{y}^\prime_m,\mathcal{Y}_k)=1$, it follows that $\|\sum_{\bm{y} \in \mathcal{Y}_k} S(\bm{y}-\bm{y}^\prime_m) \| = 0$ and the new point is said to be the {\it spatial median} of set $\mathcal{Y}_k$, i.e., it can be thought of as the ``center of mass'' of this set. Hence, the spatial depth attains the highest value of $1$ at the spatial median and decreases to zero as $\bm{y}^\prime_m$ moves away from it. The spatial depth can thus be used as a measure of ``extremeness'' of a new data point with respect to a set. In~\cite{Chen-2009}, the spatial depth of Eq.~(\ref{eq:spatial_depth}) is {\it kernelized}, which means that distances are evaluated using a positive definite kernel map. A common choice, that we also use in this paper, is the generalized Gaussian kernel $\kappa(\bm{x},\bm{y})$,
\begin{equation}
\label{eq:kernel}
\kappa(\bm{x}, \bm{y}) = \exp(-(\bm{x} - \bm{y})^T \bm{\Sigma}^{-1} (\bm{x} - \bm{y})),
\end{equation}
which provides a measure of similarity between $\bm{x}$ and $\bm{y}$. Noting that the square norm can be expressed as
\begin{equation}
\label{eq:norm}
 \left \|\bm{x}-\bm{y}\right \|^2 = \bm{x}^T\bm{x}+\bm{x}^T\bm{x}-2\bm{x}^T\bm{y},
\end{equation}
kernelizing the sample spatial depth amounts to expanding (\ref{eq:spatial_depth}) and replacing the inner products with the kernel function $\kappa$. This returns the \textit{sample KSD function} (Eq.~(4) in~\cite{Chen-2009}).\\

\noindent \textbf{Session classification procedure in an unsupervised setting:} the \ac{CNN} classifier is augmented through the detection of OOD sessions, as follows:
\begin{itemize}
\item \textit{Initialization:} for each class $k=1,\dots,K$ in the service/app identification task a number of softmax output vectors is computed by the {\it trained} \ac{CNN} using the sessions in the training set. These softmax vectors are stored in the set $\mathcal{Y}_k$. Note that, being the results of a supervised training of the \ac{CNN}, we know that the vectors in $\mathcal{Y}_k$ are all generated by a distribution that is correctly learned during the supervised training phase. 
\item \textit{Feature extraction through the \mbox{pre-trained} \ac{CNN}:} at runtime, as a new \ac{DCI} vector $\bm{x}^\prime_m$ is measured, it is inputted into the \mbox{pre-trained} \ac{CNN}, obtaining the corresponding softmax output $\bm{y}^\prime_m$.
\item \textit{Classification and OOD detection:} vector $\bm{y}^\prime_m$ is used with Eq.~(\ref{eq:kstar}) to assess the most probable class $k^\star$. At this point, Algorithm~1 of~\cite{Chen-2009} is utilized to assess whether $\bm{y}^\prime_m$ is an outlier. In case the vector is classified as an outlier, it is assigned to the OOD class, otherwise it is assigned to class $k^\star$.    
\end{itemize}
Some final remarks are in order. The outlier detection algorithm uses a threshold $t \in [0,1]$, which allows exploring the tradeoff between {\it false alarm} rate and {\it detection} rate. Instead, the covariance matrix $\bm{\Sigma}$ controls the decision boundary for rejecting vectors, driving the tradeoff between the local and global behavior of KSD. If properly chosen, the contours of KSD should closely follow those of the (actual) underlying statistical distribution. $\bm{\Sigma}$ is learned, for each class $k$, from the training vectors in $\mathcal{Y}_k$, and for the following results we picked $\bm{\Sigma} = \bm{\Sigma}_2$ in~\cite{Chen-2009}.\\

\noindent \textbf{Tuning the OOD threshold $t$:} for each class $k$, $\mathcal{S}_k$ is obtained from the training dataset. We recall that $\mathcal{S}_k$ is used to compute the covariance matrix associated with the adopted Gaussian kernel, which models the contours of the pdf of the output softmax vectors. The threshold $t \in [0,1]$ is instead used by the outlier detection algorithm to gauge the (kernelized) distance between the center of mass of set $\mathcal{S}_k$ and a new softmax vector, acquired at runtime. If $t=1$, the kernelized spatial depth of the new point will always be smaller than or equal to $t$ and all points will be rejected (marked as outliers). This is of course of no use. However, as we decrease $t$ towards $0$, we see that more and more points will be accepted, until, for $t=0$, no rejections will occur. So, $t$ determines the selectivity of the outlier detection mechanism, the higher $t$, the more selective the algorithm is. For our numerical evaluation, once the sets $\mathcal{S}_k$ are obtained for all classes $k$, we set this threshold by picking the highest value of it, $t^\star$, for which all the softmax vectors belonging to the test set are accepted, i.e., none of them is marked as an outlier (OOD). In other words, this is equivalent to making sure that the $F$-Score obtained over the test set from our trained \ac{CNN} without the OOD mechanism enabled equals that of the \ac{CNN} classifier augmented with the OOD detection capability. As $t^\star$ is the highest value of $t$ for which all the data in the test set are correctly classified as valid, our approach amounts to tuning the threshold in such a way that the outlier detection algorithm will be as selective as possible, while correctly treating all the data in the test set. In Fig.~\ref{fig:optimal_t}, we show the \mbox{$F$-Score} as a function of $t$ for the \ac{CNN} algorithm with and without OOD detection. Threshold $t^\star=0.48$ corresponds to the highest value of $t$ for which the \mbox{$F$-Score} remains at its maximum, i.e., at the end of the flat region.\\
\begin{figure}[t]
	\centering
	\includegraphics[width=.8\columnwidth]{figures/t_value}
	\caption{Finding threshold $t^\star$ using the CNN with (solid line) and without (dashed line) the OOD detection mechanism.}
	\label{fig:optimal_t}
\end{figure}

%At training time, the probability density function (pdf) $f_{\bm{y}^\prime}(\cdot)$ of the softmax output vector is estimated for each class $k=1,\dots,K$. For the following results, we did so using a Gaussian mixture, but any other approach would do. At this point, the complementary cumulative distribution function (ccdf) $F_{\bm{y}^\prime}(\cdot)$ is numerically assessed. A rejection threshold $\eta \in (0,1)$ is defined and the most probable class $k^\star$ is obtained using Eq.~(\ref{eq:kstar}). 
%At this point, a new input session $\bm{x}^\prime_m$ is marked as OOD if $F_{\bm{y}^\prime}(\bm{y}^\prime_m) \geq \eta$. This approach amount to rejecting those softmax outputs that lie within the less probable region of the pdf, i.e., whose probability of occurrence is smaller than $\eta$. 

%As an example, in Fig.~\ref{fig:cdf} we plot the cumulative distribution function (CDF) of the softmax values of \mbox{video-streaming} sessions for the labelled and unlabelled dataset. The curves are kernel density estimates from the corresponding empirical distributions. The absolute difference of the distributions can be regarded as the percentage of traffic for which the classifier has more uncertainty. For this, we calculate the Wasserstein distance~\cite{vallender1974calculation}, $d_S = \int_{-\infty}^{+\infty} |F(x)-G(x)| dx$, being $F(x)$ and $G(x)$ the distributions of softmax values obtained from the labelled and unlabelled datasets, respectively.
%\begin{equation}
%d_S = \int_{-\infty}^{+\infty} |F(x)-G(x)| dx
%\end{equation}

%\begin{figure}[h]
%	\centering
%	\includegraphics[width=\columnwidth]{figures/cdf}
%	\caption{Sample CDF (and cumulative histograms) of the CNN softmax outputs for video-streaming sessions for labelled and unlabelled data.}
%	\label{fig:cdf}
%\end{figure}

\begin{figure*}[h]
	\centering
	%	\includegraphics[width=2\columnwidth]{figures/traffic_composition_4eNB}
	%	\includegraphics[width=.48\columnwidth]
	%	{figures/campnou_composition}
	%		\includegraphics[width=.48\columnwidth]
	%	{figures/poblesec_composition}
	%		\includegraphics[width=.48\columnwidth]
	%	{figures/poblesec_composition}
	%		\includegraphics[width=.48\columnwidth]
	%	{figures/born_composition}
	%	\includegraphics[width=.48\columnwidth]
	%	{figures/bar_campnou}
	%		\includegraphics[width=.48\columnwidth]
	%	{figures/bar_campnou}
	%		\includegraphics[width=.48\columnwidth]
	%	{figures/bar_poblesec}
	%		\includegraphics[width=.48\columnwidth]
	%	{figures/bar_born}
	\includegraphics[width=.9\columnwidth]
	{figures/bar_campnou}
	\includegraphics[width=.9\columnwidth]
	{figures/bar_cttc}
	\includegraphics[width=.9\columnwidth]
	{figures/bar_poblesec}
	\includegraphics[width=.9\columnwidth]
	{figures/bar_born}
	\caption{Traffic decomposition at service level for the four monitored \acp{eNodeB} during the $24$ hours of a day.}
	\label{fig:traffic_composition}
\end{figure*}


\noindent \textbf{Experimental analysis of \ac{eNodeB} traffic:} in Fig.~\ref{fig:traffic_composition}, the traffic decomposition into the considered service classes is shown for the four selected \acp{eNodeB} using $t^\star=0.48$. The percentage of sessions identified as OOD, for which the classifier is uncertain, is also reported at the top of each bar.
%This is computed for each of the 2-hours time-slot $S$, $S=1,\dots,12$, and the average value is shown and labelled as \textit{OOD} in the traffic composition in Fig.~\ref{fig:traffic_composition}, to include other typologies of services.
Common characteristics are observed in all the considered deployments:
\begin{itemize}
	\item the most used service is \mbox{video-streaming}, with typical shares ranging from $50\%$ to $80\%$. This confirms the measurements in~\cite{ericsson} and~\cite{ciscovni}.
	\item The least used service is \mbox{video-call}, whose share is typically between $5\%$ and $10\%$, whereas \mbox{audio-streaming} takes $21\%$ of the total traffic load.
	\item OOD sessions are consistently well below $8\%$. Note that this share accounts for all those apps that are not tracked by our classifier, such as texting, web browsing, and file transfers. 
\end{itemize}

Through the proposed service identification approach, we can accurately characterize, at runtime, the used services. Moreover, the traffic decomposition at service level allows one to make some interesting considerations on the land use. For example, in a typical residential area (PobleSec) the \mbox{audio-streaming} service is the one used the least across the four monitored sites, with an average of $16.4\%$. Instead, in a typical office and university neighborhood (Castelldefels), \mbox{audio-streaming} has the highest traffic share across all sites ($22\%$ on average). Born and CampNou, which are two leisure districts, present a similar traffic distribution across the day.  We finally remark that, while the traffic profiling results are shown using a time granularity of one hour, our classification tool allows for traffic decomposition at much shorter timescales, i.e., on a \mbox{per-session} basis.

%\subsection{Traffic Characterization during Match Days}
%As highlighted in the Section~\ref{sec:dataset}, one of the monitored eNodeBs is located close to Camp Nou, a popular football stadium in Barcelona, that hosts on average 77000 people during match day\cite{}. By analyzing the traffic during such event, we are able to retrieve significant information on how the network mobile needs to adjust to support such intense traffic increment. In Fig.~\ref{fig:campnou_aggregate}, we can observe the downlink aggregated traffic of the monitored eNodeB. In particular, during the match time, we can see traffic peaks that are $2.3$ higher than the average traffic and about $1.3$ times higher than the average daily peaks.
%
%As done in the previous use case, using the pre-trained classifiers we are able to classify the single user sessions during this time interval, and retrieve the traffic characterization of the mobile user traffic. The traffic composition of the 3 datasets are shown in Fig.~\ref{fig:matches_composition}. The first two datasets are collected during match days, within a slot of $2$ hours, that comprises the match time. These two measurements are compared to another user sessions' dataset, collected during a time slot when no sport events are scheduled. The bar plots in Fig.~\ref{fig:matches_composition}, gives the composition in percentage of the mobile traffic among the three type of services that we account in our study. Moreover, the absolute values of the three bars show that the traffic segmentation is similar during such events (with an average difference minor than $6\%$), and the eNodeB faces a two times increment of the traffic volume with respect to the traffic generated when no matches are scheduled. These results validate the performed service classification: during the matches the traffic segmentation is similar and video-streaming applications dominate the distribution of traffic, while video-calls are significantly reduced with respect to the case of no match. This is aligned with expected social behaviours.
%\begin{figure}[t]
%\centering
%\includegraphics[width=\columnwidth]{figures/campnou_aggregate}
%\caption{A snapshot of the Downlink Aggregated Traffic of the Camp Nou traces. The time resolution is $25$ minutes.}
%\label{fig:campnou_aggregate}
%\end{figure}
%\begin{figure}[h!]
%\centering
%\includegraphics[width=\columnwidth]{figures/matches_composition}
%\caption{Traffic composition by service during match and no-match events.}
%\label{fig:matches_composition}
%\end{figure} 

==> Neural_Networks.tex <==
%!TEX root = main.tex

\section{Neural Networks}
\label{sec:nn}

In this section, we present three approaches based on neural networks used for the traffic classification problem. Specifically, we have employed a \ac{MLP}, a \ac{RNN} network and a \ac{CNN}. Details about the customized architectures are provided hereafter. It should be noted that the layer settings provided for each \ac{NN} are specific for the obtained dataset explained in Section~\ref{sec:dataset}, with the goal of obtaining the highest performance in terms of accuracy, with the lowest complexity. In contrast to previous methods presented in Section~\ref{sec:sl}, these tools enable automatic feature detection within the raw dataset traces, which provides an improvement in the classification performance as we will show shortly in Section~\ref{sec:results}.

\subsection{Multilayer Perceptron}
\label{sec:nn_mlp}
A multilayer perceptron is a \mbox{feed-forward} (the input signal goes only one way within the network) artificial neural network  that generates a set of outputs from a set of inputs. An MLP is characterized by, at least, three layers of nodes: an input, a hidden layer and an output, and these layers are connected as a directed graph between the input and output layers. Except for the input nodes, each node is a neuron that uses a nonlinear activation function to produce an output. MLP utilizes a supervised learning technique called backpropagation for training, i.e., to find the weights for each neuron within the network that minimize a certain error objective function. It can distinguish data that is not linearly separable. For further details, please refer to \cite{bishop2006}.

In the present work, the customized \ac{MLP} architecture we have used for the classification is composed by three fully connected layers. Details are as follows. First, an input layer ${MLP}_1$ with $N_{{MLP}_1}= 128$ neurons is used, where each neuron uses a leaky version of a \ac{ReLU}. The ReLU activation function is used a lot in neural network architectures and allows the activation to be thresholded at zero. However, during the training, large gradient flows through a ReLU neuron can cause the weights to update in such a way that the neuron will never activate on any data point again. If this happens, then the gradient flowing through the unit will forever be zero from that point on, and the neuron will be useless. Leaky \acp{ReLU} attempt to solve this, by forcing the function to have a small negative slope rather than zero value. The leaky \ac{ReLU} activation function has been used due to the need of tackling \mbox{non-linearities} present in the dataset. Given an input $x$, it is defined as follows:
%
\begin{equation}
	f(x) = \left\{ 	\begin{array}{lr} 	\alpha x & : x < 0\\ 	x & : x \ge 0 	\end{array} \right.
\end{equation}

\noindent where $\alpha$ controls the negative slope and usually takes values around $0.1$.
Moreover, the use of only linear activation functions in every layer would imply that the final activation function of the last layer would be just a linear function of the first layer input. This means that several layers can be replaced by a single layer, losing the ability of stacking layers and its improvement in finding hidden features within the input dataset.
Then, there is a second fully connected layer ${MLP}_2$, i.e., each output neuron is connected to all input neurons of this layer (weights are not shared), that comprises $N_{{MLP}_2}= 64$ neurons with the same activation function as the first one. Finally, each output neuron in the last layer ${MLP}_3$ corresponds to a specific class $k \in K$, where $K=6$ classes for app classification and $K=3$ for service classification. 

The output vectors of all layers have binary entries and are \mbox{hot-encoded}, i.e., all values are zero except for the entry corresponding to the output chosen class. The output of layer ${MLP}_3$ is a stochastic vector $\bm{y}$ obtained by a softmax activation function, whose $k$-th entry $k = 1,2,\dots,K$ can be seen as the probability that the input pattern belongs to class $k$, i.e., $y_k = y_k(\bm{w},\bm{X}) = Prob(t_k = 1|\bm{w},\bm{X})$, where $\bm{w}$ is the vector containing all the \ac{MLP} weights, $\bm{X}$ is the current input matrix and $t_k = 1$ if $\bm{X}$ belongs to class $k$ and $t_k = 0$ otherwise. If $\bm{X}$ is the set of all training examples, we define the batch set as $\mathcal{B} \subset \mathcal{X}$. Let $\bm{X} \in \bm{B}$ and denote the corresponding output vector by $\bm{y}(\bm{w},\bm{X})$ and its $k$-th entry by $y_k(\bm{w},\bm{X})$. The corresponding target vector is $\bm{t(X)} = (t_1(\bm{X}), \dots, t_k(\bm{X}))^T$ \cite{gadaleta2016idnet}. The network is trained in a supervised manner solving a \mbox{multi-class} classification problem using the {\it RMSprop} algorithm~\cite{tieleman2012lecture}, a specific gradient descend algorithm which minimizes a categorical \mbox{cross-entropy} loss function $L(\bm{w})$, defined as \cite{bishop2006} (Eq. (5.24) of Section 5.2):

\begin{equation}
\label{eq:cross}
	L(\bm{w}) = - \sum_{\bm{X} \in \bm{B}} \sum_{k=1}^{K} t_k(\bm{X}) log(y_k(\bm{w},\bm{X})).
\end{equation}

During training, Eq.~\ref{eq:cross} is iteratively minimized, by rotating training examples in the batch set $\mathcal{B}$ so as to span the entire input set $\mathcal{X}$. 

\subsection{Recurrent Neural Network}
\label{sec:nn_rnn}
\ac{RNN} are a generalization of feedforward neural networks, that have been devised for handling temporal and predictive problems. \ac{LSTM} networks are a particular kind of \ac{RNN}, introduced in \cite{Hochreiter1997}. They have been explicitly designed to avoid the \mbox{long-term} dependency issue, which is the cause of the \mbox{vanishing-gradient} problem in normal \acp{RNN} \cite{gers1999learning}.

The capability of learning \mbox{long-term} dependencies is due to the structure of the \ac{LSTM} units, which incorporates gates that regulate the learning process. The neurons in the hidden layers of an \ac{LSTM} are \acp{MC}. A \ac{MC} has the ability to store or forget information about past network states by using structures called {\it gates}, which consist of a cascade of a neuron with sigmoidal activation function and a pointwise multiplication block. Thanks to this architecture, the output of each memory cell possibly depends on the entire sequence of past states, making \acp{LSTM} suitable for processing time series with long time dependencies~\cite{Hochreiter1997}. An \ac{LSTM} memory cell diagram is presented in Fig.~\ref{fig:lstm_diagram}. The input gate is a neuron with sigmoidal activation function ($\sigma$). Its output determines the fraction of the MC input that is fed to the cell state block. Similarly, the forget gate processes the information that is recurrently fed back into the cell state block. The output gate, instead, determines the fraction of the cell state output that is to be used as output of the MC at each time step. Gate neurons usually have sigmoidal activation functions ($\sigma$), while the input and cell state use the hyperbolic tangent ($\tanh$) activation function. All the internal connections of the \ac{MC} have unitary weight~\cite{Hochreiter1997}.

\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{figures/lstm_cell.eps}
	\caption{\ac{LSTM} memory cell diagram.}
	\label{fig:lstm_diagram}
\end{figure} 

\begin{figure}[t]	
	\centering
	\includegraphics[width=\columnwidth]{figures/lstm.eps}
	\caption{\ac{RNN} architecture.}
	\label{fig:lstm_nn}	
\end{figure}

The proposed architecture for the traffic classification is depicted in Fig.~\ref{fig:lstm_nn}. In our design, we consider three stacked layers combining two LSTM layers with a final output fully connected layer. The first layer ${RNN}_1$ is composed by $N_{{RNN}_1}= 180$ \acp{MC} and the second one ${RNN}_2$ has $N_{{RNN}_2}= 180$ as well. The final fully connected layer ${RNN}_3$ performs the actual \mbox{multi-class} classification as the final layer in the \ac{MLP} network. Hence, the explanation given in \ref{sec:nn_mlp} about it also applies here. Moroever, the same optimizer to minimize Eq.~\ref{eq:cross} has been used in this case.

\subsection{Convolutional Neural Network}
\label{sec:nn_cnn}

\acp{CNN} are \mbox{feed-forward} deep neural networks differing from fully connected multilayer networks for the presence of one or more convolutional layers. At each convolutional layer, a number of kernels is defined. Each of them has a number of weights, which are convolved with the input in a way that the same set of weights, i.e., the same kernel, is applied to all the input data, moving the convolution operation across the input span. Note that, as the same weights are reused (shared weights), and each kernel operates on a small portion of the input signal, it follows that the network connectivity structure is sparse. This leads to advantages such as a considerably reduced computational complexity with respect to fully connected feed forward neural
networks \cite{gadaleta2016idnet}. For more details the reader is referred to \cite{goodfellow2016deep}. CNNs have been proven to be excellent feature extractors for images \cite{gadaleta2016idnet} and here we prove their effectiveness for mobile traffic data. 

The \ac{CNN} architecture that we designed to this purpose is shown in Fig.~\ref{fig:cnn}. It is composed of a cascade of two convolutional layers, followed by a pooling layer respectively, and finally a  \mbox{two-layer} fully connected network. The convolutional layers in combination with the first fully connected layer perform a dimensionality reduction (or automatic feature extraction) task, whereas the last fully connected one performs the \mbox{multi-class} classification. The first convolutional layer $CNN_1$ uses one dimensional kernels ($1$x$5$ samples) performing a first filtering of the input and processing each input vector (rows of $\bm{X}$) separately. The activation functions are linear and the number of convolutional kernels is referred to as $N_{{CNN}_1}=32$. 
The second convolutional layer $CNN_2$ uses again one dimensional kernels ($1x5$ samples) with  non-linear hyperbolic tangents as activation functions, and the number of convolutional kernels is referred to as $N_{{CNN}_2}=64$.
Max pooling is applied to the output of $CNN_1$ and $CNN_2$ to further reduce its dimensionality and increase the spatial invariance of features \cite{gadaleta2016idnet}. In both cases, a \mbox{one-dimensional} pooling with kernel $1$x$3$ is performed. Finally, th fully connected network is composed of two layers. The first one $CNN_3$ helps in finding hidden features from the input data and has $N_{{CNN}_2}=32$ neurons with leaky \ac{ReLU} activation function. It has been added to reduce computation time while achieving the same accuracy as compared with the case where a third convolutional layer was added. The final output layer $CNN_4$ follows the same architecture as previously mentioned (see last paragraph of Section~\ref{sec:nn_mlp}).

\begin{figure}[t]	
	\centering
	\includegraphics[width=\columnwidth]{figures/cnn.eps}
	\caption{\ac{CNN} architecture.}
	\label{fig:cnn}	
\end{figure}


==> Supervised_Learning_Approach.tex <==
%!TEX root = main.tex

\section{Supervised Learning}
\label{sec:sl}

In this section, we present several supervised \ac{ML} algorithms that are used as benchmarks for the two classification problems: for the sake of clarity, we distinguish two classes of classification algorithms, whether they include a \mbox{\ac{NN}-based} structure or not. Details about the \mbox{\ac{NN}-based ones} are given in Section~\ref{sec:nn}. The other group of classifiers are presented as follows. 

\subsection{Linear Classifiers}
For this type of algorithms, we choose a linear \ac{SVM} and logistic regression. Both are discriminative models, which means that they try to model by just depending on the observed data while learning how to do the classification. Unlike generative models, a discriminative model makes fewer assumptions on the distributions but depends heavily on the quality of the data. 

Generally, given a linear classifier, if the input feature vector is ${\bm{x}}$, then the output score  is: 
\begin{equation}
\bm{y}=f({\bm{w}}\cdot {\bm {x}})=f\left(\sum _{j}w_{j}x_{j}\right)
\end{equation}	

\subsubsection{Linear Logistic Regression} Although this algorithm derives from linear regression, it can be used to perform classification. In linear regression, the output  is modeled as a linear combination of features: $\bm{y} = \sum _{j}w_{j}x_{j} + b$. Differently, in logistic regression, in a binary case, is the probability of the output that is modeled as a linear combination of the features. The following is also called Logit function: 
\begin{equation}
log\left(\frac{\pi}{1-\pi}\right) = \sum _{j}w_{j}x_{j}+b
\end{equation}

where $\pi$, in a binary case, is the probability of $\bm{x}$ to belong to one of the two class. It follows that $\pi$ is given by:
\begin{equation}
\pi = \frac{e^{\sum _{j}w_{j}x_{j} + b}}{1+e^{\sum _{j}w_{j}x_{j} + b}}=
\frac{1}{1+e^{-{\sum _{j}w_{j}x_{j} + b}}},
\end{equation}
which is the Logistic function. For this reason, this classifier represents a particular case of a linear model, since it is the probability of belonging to a class that is modeled as a linear combination and not the actual output. In our problem, we adopt the implementation from the library presented in~\cite{fan2008liblinear}.

\subsubsection{Linear SVM} Support vector machines defines hyperplanes to separate the input data in the features vector space, maximizing the margin around the separating hyperplane. The decision function is fully specified by a small subset of training samples, the support vectors. 

In our problem, we use a linear SVM classifier to identify the different mobile apps. In our implementation, we use the Hinge loss function~\cite{wu2007robust} to compute the \mbox{maximum-margin} classification. We use a standard L2-norm for regularization with the penalty parameter $C=0.025$. The library implementation details can be found here\cite{chang2011libsvm}.
% For the loss, we use the Hinge loss function \angel{(Add ref here)} to compute the \mbox{maximum-margin} classification.
%\begin{equation}
%L(y)=\max(0,1-t\cdot y)
%\end{equation}
%where $y$ is the classifier score and $t\in \left(0,1\right)$ is the intended output. 
\mbox{Non-linear} SVM can be implemented by applying a kernel function instead of the matrix multiplication, but the kernel selection and the analysis to obtain non linearities deserves a separate study. \\


Both linear methods are originally intended for binary classification, but the extension from the binary case to a \mbox{multi-class} classification can be done using the \mbox{one-vs-all} scheme~\cite{fan2008liblinear}.

\subsection{Random Forest} Random forest is an ensemble learning method, which operates by constructing a multitude of decision trees at training time, and outputting the predicted class, i.e., service or app type, of the input user session. With respect to larger decision trees, random forests are less prone to overfitting over the training dataset. Thus, random forests are used to average multiple deep decision trees, with the goal of reducing the variance, generally boosting the accuracy in the final model.

Formally, the random forest consists of a collection of tree-structured classifiers $h(\bm{X},\theta_{n_t})$ with $n_t=1, ..., N_T$, $N_T$ number of trees, and $\theta_{n_t}$ are independent identically distributed random vectors, which account for the random choices we make when fitting the $n_t$-th tree~\cite{breiman2001random}. In our work, we choose $N_T=10$ and we use the bootstrap technique (also known as \textit{bagging}) for the random choices. Given $M$ the total number of sessions, $\bm{y}$ the output class vector and $N_T$ the total number of trees, the bagging technique for random sampling applies as follows:
\begin{algorithm}[h]
\SetAlCapSkip{2em}
 \For{$n_t = 1 \dots N_T$}{
 {
 \begin{itemize}[leftmargin=*]{
 \itemsep0.5em 
  \item sample, with replacement, $M$ training examples from $\bm{X}, \bm{y}$; these are $X_{n_t}, \bm{y}_{n_t}$\;
  \item train the classification tree $h(\bm{X},\theta_{n_t})$ on  $X_{n_t}, \bm{y}_{n_t}$\; 
 }
 \end{itemize}
  }
 }
 \caption{Bootstrap procedure for random forests.}
\end{algorithm}

\subsection{Gaussian Processes} 
%Bayesian \mbox{non-parametric} models, such as Gaussian Processes (GPs), can represent beliefs about the model parameters via a probability distribution (called the {\it prior} distribution). Then, Bayesian inference can reshape the prior distribution, transforming it into a {\it posterior} one. GPs have become popular for regression and classification, often showing impressive empirical performance.

%A GP is a generalization of the Gaussian probability distribution and can be used for probabilistic classification. Formally, a GP is a collection of random variables, any finite number of which have a joint Gaussian distribution and it is completely specified by the mean function $m(x)$ and the covariance function $k(x, \hat x)$ .
%\begin{equation}f(\cdot) \sim GP(m(x), k(x, \hat x))\end{equation} 


%For a binary classification task, we need to predict the probability $\pi(x)$, which lies in $[0,1]$:  the basic idea behind the Gaussian process prediction is to place a GP prior over the latent function $f(x)$ and then squash $f(x)$ through any sigmoid function to obtain a prior on $\pi(x) = \sigma(f(x))$. The latent function is a so-called nuisance function, whose values are not observed and are not relevant by themselves. Its purpose is to allow a convenient formulation of the model, and  is removed during prediction. Generally, the Logistic function is used to squash $f(x)$.

%In contrast to a regression task, the posterior of the latent function $\pi(x)$ is not Gaussian even for a GP prior because of discrete class labels. Rather, a non-Gaussian likelihood corresponding to the logistic function is used. The approximation of the non-Gaussian posterior with a Gaussian likelihood is done by using the Laplace approximation. The details of the GP implementation can be found in~\cite{rasmussen2004gaussian}.

Gaussian Processes (GPs) are a \mbox{non-parametric} approach that aims to find a distribution over all the possible functions $f(x)$ that are consistent with the observed data. As with all Bayesian methods, it begins with a prior distribution which is updated as data points are observed, producing the posterior distribution over functions.

Although to represent a distribution over a set of possible functions can be difficult, it turns out that only a distribution over the function's values at a finite, but arbitrary, set of points is needed. Formally, a GP is a collection of random variables, any finite number of which have a joint Gaussian distribution and it is completely specified by the mean $\mu(x)$ and covariance function $\Sigma(x)$:

\begin{equation}
f(\cdot) \sim GP(\mu(x), \Sigma(x)).
\end{equation} 

As described in~\cite{rasmussen2004gaussian}, GPs can be used for classification tasks, finding a probability $\pi(x)$ that lies in $[0,1]$: the basic idea behind is to place a prior Gaussian distribution over the latent function $f(x)$ and then squash $f(x)$ through any sigmoid function to obtain a prior on $\pi(x) = \sigma(f(x))$. The latent function is a \mbox{so-called} nuisance function, whose values are not observed and are not relevant by themselves. Its purpose is to allow a convenient formulation of the model, and is removed during prediction. In our work, the Logistic function is used to squash $f(x)$. The details of the GP implementation can be found in~\cite{rasmussen2004gaussian}.


==> new_table.tex <==
%%!TEX root = main.tex
\begin{table*}[t]
\centering
\ra{0.7}
\trinh{

\begin{tabular}{*{8}{c}}\toprule

\textbf{Algorithm}&\multicolumn{1}{c}{\textbf{Accuracy $\%$}} & \multicolumn{1}{r}{\textbf{Precision}} & \textbf{Recall} & \textbf{F-Score} & \textbf{\# Parameters}  & \textbf{Acc Async $\%$} & \textbf{Diff $\%$} \\
\midrule
\rowcolor{black!5} Linear SVM & 80.07 & 0.815 & 0.801 & 0.801   & 36726 & 64.34 & -15.8\\
\rowcolor{black!0}Logistic Regressor & 74.84 & 0.741 & 0.748  & 0.748   &  486 & 63.23 & -11.6 \\
\rowcolor{black!5}Nearest Neighbours   & 77.78 & 0.797 & 0.778  & 0.778   &   36720 & 76.56 & -1.2 \\
\rowcolor{black!0}Random Forest  & 77.12 & 0.813 & 0.771  & 0.760   &   41310 & 68.41 & -8.7\\
\rowcolor{black!5}Gaussian Processes  & 86.93 & 0.873 & 0.869  & 0.869   &   146720 & 79.08 & -7.8\\
\midrule
\textbf{Neural Networks} &  &   &    &    &  \\
\midrule
\rowcolor{black!5}MLP & 86.27 & 0.866  &  0.863  & 0.860  &  19014 & 81.16 & -5.1 \\
\rowcolor{black!0} RNN  &  95.37 & 0.956  & 0.954   & 0.954  & 392046  & 90.05 & -5.3\\
\rowcolor{black!5}CNN & 97.83 & 0.978 & 0.978  & 0.978   & 25062 & 91.48 & -6.4\\
\bottomrule

\end{tabular}
}
\caption{Classifiers comparison for the app identification task.}
\label{table_app}
\end{table*}




==> new_table2.tex <==
%!TEX root = main.tex
\begin{table*}[t]
\centering
\ra{0.7}
\trinh{

\begin{tabular}{*{8}{c}}\toprule

\textbf{Algorithm}&\multicolumn{1}{c}{\textbf{Accuracy $\%$}} & \multicolumn{1}{r}{\textbf{Precision}} & \textbf{Recall} & \textbf{F-Score} & \textbf{\# Parameters} & \textbf{Acc Async $\%$} & \textbf{Diff $\%$} \\
\midrule
\rowcolor{black!5} Linear SVM & 87.58 & 0.877 &  0.875 & 0.871  &  19843 & 78.51  & -9.0\\
\rowcolor{black!0}Logistic Regressor & 87.58 & 0.883 & 0.875 & 0.877   & 243 & 79.28 & -8.3\\
\rowcolor{black!5}Nearest Neighbours   & 82.67 & 0.850 & 0.826 & 0.833 &  19840 & 81.56 & -1.1\\
\rowcolor{black!0}Random Forest  & 89.54 & 0.915 & 0.895 & 0.901 &  22320 & 81.27 & -8.3\\
\rowcolor{black!5}Gaussian Processes  &  92.81 & 0.932 & 0.928 & 0.928 &  73360 & 80.78 & -12.0\\
\midrule
\textbf{Neural Networks} &  &   &    &    & \\
\midrule
\rowcolor{black!5}MLP &  92.81 & 0.930 & 0.928 & 0.929  & 18819 & 91.31 & -1.5 \\
\rowcolor{black!0} RNN  &  98.14 & 0.981 & 0.982 & 0.981 & 391503 & 94.46 & -3.7\\
\rowcolor{black!5}CNN & 99.07 & 0.986 & 0.994 & 0.989  & 24963 & 95.39 & -3.7\\
\bottomrule
\end{tabular}
}
\caption{Classifiers comparison for the service identification task.}
\label{table_service}

\end{table*}

==> table.tex <==
%%!TEX root = main.tex
\begin{table*}[t]
\centering
\ra{0.7}

\begin{tabular}{*{6}{c}}\toprule
\textbf{Algorithm}&\multicolumn{1}{c}{\textbf{Accuracy $\%$}} & \multicolumn{1}{r}{\textbf{Precision}} & \textbf{Recall} & \textbf{F-Score} & \textbf{\# Parameters}  \\
\midrule
\rowcolor{black!5} Linear SVM & 80.07 & 0.815 & 0.801 & 0.801   & 36726 \\
\rowcolor{black!0}Logistic Regressor & 74.84 & 0.741 & 0.748  & 0.748   &  486 \\
\rowcolor{black!5}Nearest Neighbours   & 77.78 & 0.797 & 0.778  & 0.778   &   36720\\
\rowcolor{black!0}Random Forest  & 77.12 & 0.813 & 0.771  & 0.760   &   41310\\
\rowcolor{black!5}Gaussian Processes  & 86.93 & 0.873 & 0.869  & 0.869   &   146720\\
\midrule
\textbf{Neural Networks} &  &   &    &    &  \\
\midrule
\rowcolor{black!5}MLP & 86.27 & 0.866  &  0.863  & 0.860  &  19014  \\
\rowcolor{black!0} RNN  &  95.37 & 0.956  & 0.954   & 0.954  & 392046  \\
\rowcolor{black!5}CNN & 97.83 & 0.978 & 0.978  & 0.978   & 25062 \\
\bottomrule
\end{tabular}
\caption{Classifiers comparison for the app identification task.}
\label{table_app}
\end{table*}




==> table2.tex <==
%!TEX root = main.tex
\begin{table*}[t]
\centering
\ra{0.7}

\begin{tabular}{*{6}{c}}\toprule
\textbf{Algorithm}&\multicolumn{1}{c}{\textbf{Accuracy $\%$}} & \multicolumn{1}{r}{\textbf{Precision}} & \textbf{Recall} & \textbf{F-Score} & \textbf{\# Parameters} \\
\midrule
\rowcolor{black!5} Linear SVM & 87.58 & 0.877 &  0.875 & 0.871  &  19843\\
\rowcolor{black!0}Logistic Regressor & 87.58 & 0.883 & 0.875 & 0.877   & 243\\
\rowcolor{black!5}Nearest Neighbours   & 82.67 & 0.850 & 0.826 & 0.833 &  19840\\
\rowcolor{black!0}Random Forest  & 89.54 & 0.915 & 0.895 & 0.901 &  22320\\
\rowcolor{black!5}Gaussian Processes  &  92.81 & 0.932 & 0.928 & 0.928 &  73360\\
\midrule
\textbf{Neural Networks} &  &   &    &    & \\
\midrule
\rowcolor{black!5}MLP &  92.81 & 0.930 & 0.928 & 0.929  & 18819  \\
\rowcolor{black!0} RNN  &  98.14 & 0.981 & 0.982 & 0.981 & 391503 \\
\rowcolor{black!5}CNN & 99.07 & 0.986 & 0.994 & 0.989  & 24963\\
\bottomrule
\end{tabular}
\caption{Classifiers comparison for the service identification task.}
\label{table_service}
\end{table*}
